SYGMA: System for Generalizable Modular Question Answering OverKnowledge Bases

Knowledge Base Question Answering (KBQA) tasks that in-volve complex reasoning are emerging as an important re-search direction. However, most KBQA systems struggle withgeneralizability, particularly on two dimensions: (a) acrossmultiple reasoning types where both datasets and systems haveprimarily focused on multi-hop reasoning, and (b) across mul-tiple knowledge bases, where KBQA approaches are specif-ically tuned to a single knowledge base. In this paper, wepresent SYGMA, a modular approach facilitating general-izability across multiple knowledge bases and multiple rea-soning types. Specifically, SYGMA contains three high levelmodules: 1) KB-agnostic question understanding module thatis common across KBs 2) Rules to support additional reason-ing types and 3) KB-specific question mapping and answeringmodule to address the KB-specific aspects of the answer ex-traction. We demonstrate effectiveness of our system by evalu-ating on datasets belonging to two distinct knowledge bases,DBpedia and Wikidata. In addition, to demonstrate extensi-bility to additional reasoning types we evaluate on multi-hopreasoning datasets and a new Temporal KBQA benchmarkdataset on Wikidata, namedTempQA-WD1, introduced in thispaper. We show that our generalizable approach has bettercompetetive performance on multiple datasets on DBpediaand Wikidata that requires both multi-hop and temporal rea-soning

==> TempQA-AAAI2022(2)/text/abstract.tex <==
\begin{abstract}
 
 Knowledge Base Question Answering (KBQA) tasks that involve complex reasoning are emerging as an important research direction. However, most of the recent KBQA systems are built towards supporting multi-hop reasoning over a single knowledge base. In this paper, we present a KBQA system that is built with the goal of generalizing across multiple knowledge bases and multiple reasoning types. Our system built as modular pipeline, by keeping interpretability at intermediate stages also as the guiding principle, contains three high level modules: 1) KB-agnostic question understanding module that is common across KBs 2) Ontology module to support additional reasoning types simply by extending the ontology and 3) KB-specific question mapping and answering module to address the KB specific aspects of the answer extraction. We demonstrate effectiveness of our system by evaluating on datasets belonging to two distinct knowledge bases, DBpedia and Wikidata. In addition, to demonstrate extensibility to additional reasoning types we evaluate on a new Temporal KBQA benchmark dataset, named TempQA-WD, introduced in this paper. This dataset is adapted from an old dataset to Wikidata. We show state-of-the-art results achieved on DBpedia based LCQuad and QALD datasets and Wikidata based WebQSP datasets. Additionally, we also present baseline numbers achieved on the new temporal dataset.
 
 %Question Answering of Knowledge Bases has been a long standing problem in the Natural Language Processing domain. The goal of the task is to evaluate systems ability to reason and retrieve an answer from the knowledge base, given the natural language question. 
 
 %Knowledge Base Question Answering (KBQA) tasks that involve complex reasoning are emerging as an important research direction. However, most existing KBQA datasets focus primarily on generic multi-hop reasoning over explicit facts, largely ignoring other reasoning types such as temporal, spatial, and taxonomic reasoning. In this paper, we present a benchmark dataset for temporal reasoning, \dataset, to encourage research in extending the present approaches to target a more challenging set of complex reasoning tasks. Specifically, our benchmark is a temporal question answering dataset with the following advantages: (a) it is based on Wikidata, which is the most frequently curated, openly available knowledge base, (b) it includes intermediate sparql queries to facilitate the evaluation of semantic parsing based approaches for KBQA, and (c) it generalizes to multiple knowledge bases: Freebase and Wikidata. %allows evaluating generalizable temporal KBQA systems on multiple knowledge bases (Freebase and Wikidata);  
 %Including the dataset, we present a modular temporal knowledge base question answering system on Wikidata as a baseline system. Overall, the baseline system shows a performance of XX on the dataset showing significant headroom for research in the temporal reasoning domain.
 %In addition to the new dataset, we present a modular, temporal KBQA system  \system~as a baseline. Overall, the baseline system shows a performance of 0.32 (F1 metric) on the dataset showing significant headroom for research in the temporal reasoning domain.
 
 
 %(b) they target only one knowledge base lacking the ability for the systems to show generalized approaches over multiple knowledge bases; (c) most datasets have question-answer pairs without an intermediate SPARQL representation. \pavan{Both b and c are primarily for Temporal Question Answering.}


 %We describe a benchmark dataset that we release towards facilitating effective evaluation of approaches, and to try address gaps in the existing benchmarks. Our main goal with this dataset is to encourage approaches that are interpretable and generalizable across different knowledge bases and reasoning requirements. In specific, we took an existing temporal question answering (QA) dataset that was built for Freebase and adapted a subset of that to build a parallel dataset for Wikidata. This enables performance evaluation of temporal KBQA approaches simultaneously on more than one knowledge base. In addition we also provide fine-grained annotation on a subset that enable evaluating interpretability of the approach. Apart from the dataset, we also present a neuro-symbolic approach for temporal KBQA that could serve as a baseline approach on this dataset. This approach includes a question understanding framework where an intermediate KB-agnostic logic representation of the question is obtained first, followed by mapping onto a KB-specific logic representation that further could be executed over KB after mapping onto corresponding SPARQL queries. {\pavan{Pavan: 1. KBQA datasets lacks reasoning with most datasets primarily focused on multi-hop reasoning. Need to including more reasoning types for extending research in KBQA. 2. KBQA datasets cover single knowledge bases. There is a need for parallel datasets that can help evaluate generality of approaches on multiple datasets. 3. KBQA datasets with weak supervision push approaches to directly work with the knowledge graph. Having an intermeditate representation such as a SPARQL query would encourage KG-generic semantic parsing.}}
\end{abstract}

==> TempQA-AAAI2022(2)/text/abstract_pavan.tex <==
\begin{abstract}
 
Knowledge Base Question Answering (KBQA) tasks that involve complex reasoning are emerging as an important research direction. However, most KBQA systems struggle with generalizability, particularly on two dimensions: (a) across multiple reasoning types where both datasets and systems have primarily focused on multi-hop reasoning, and (b) across multiple knowledge bases, where KBQA approaches are specifically tuned to a single knowledge base. In this paper, we present \system, a modular approach facilitating generalizability  across multiple knowledge bases and multiple reasoning types. Specifically, \system~contains three high level modules: 1) KB-agnostic question understanding module that is common across KBs 2) Rules to support additional reasoning types and 3) KB-specific question mapping and answering module to address the KB-specific aspects of the answer extraction. We demonstrate effectiveness of our system by evaluating on datasets belonging to two distinct knowledge bases, DBpedia and Wikidata. In addition, to demonstrate extensibility to additional reasoning types we evaluate on multi-hop reasoning datasets and a new Temporal KBQA benchmark dataset on Wikidata, named \dataset\footnote{https://github.com/IBM/tempqa-wd}, introduced in this paper. We show that our generalizable approach has better competetive performance on multiple datasets on DBpedia and Wikidata that requires both multi-hop and temporal reasoning. %Additionally, we also present baseline numbers achieved on the new temporal dataset.
 
 
\end{abstract}

==> TempQA-AAAI2022(2)/text/approach.tex <==
\section{~\system: System Description}
\label{sec:baseline}
Motivated by \citet{pavan2020},~\system~is designed as a neuro-symbolic system, avoiding the need for end-to-end training. Figure \ref{fig:pipeline} shows the overall KBQA pipeline with independent modules and their intermediate representations. The approach is designed with the goal of generalization across multiple KBs and reasoning types. Supporting generalization is accomplished in two stages as shown in Figure~\ref{fig:pipeline},  driven by an example in Figure~\ref{fig:example}. The first is a \textit{KB-agnostic question understanding} stage, which takes in a natural language question as input and outputs an intermediate  representation that can be common across different KBs. The second is \textit{question mapping and reasoning} stage where, first, the necessary heuristics to introduce templates for new reasoning types are applied. Next, the KB-agnostic representation is mapped to the vocabulary of the KG to output KB-specific representation that has a deterministic mapping to SPARQL. We use Wikidata and DBpedia to show generalization across KBs, and use multi-hop and temporal reasoning to evaluate across reasoning types.  
% Figure~\ref{fig:pipeline} shows the modules in each of the stages and Figure \ref{fig:example} demonstrates these modules and its intermediate representations with an example. 
Before we get into the details of these modules and intermediate representations, we give a brief description of the Lambda calculus and the temporal functions used by \system\ to generate its intermediate logic representation.
%and KB Specific question mapping and reasoning module to handle KB specific aspects. Extensible support for adding new reasoning types is handled by the KB-Agnostic rules and KB-Specific-Rules that are utilized by the pipeline to easily add new reasoning templates to the system.
\begin{figure*}[t!]
  \centering
  \includegraphics[width=0.9\linewidth]{./figures/SystemArchitecture_2}
  %\includegraphics{./figures/pipeline}
  \caption{Architecture of ~\system\ that shows the pipeline with independent modules and intermediate representations. The intermediate representations are supported by appropriate heuristics to facilitate generalizability.}
  \label{fig:pipeline} 
\end{figure*}

%Our system is built as a stack of modules, that transforms questions along the pipeline step-by-step through intermediate representations, that gradually takes them closer to the representation matching the underlying KB. \mdc{re-word}  The temporal question has two events as color coded in blue and red in the lambda expression along with required interval operators to get the required time intervals for both events and the temporal constraint overlap color coded in green color. How we add these additional temporal reasoning operators into the system using AMR representation is discussed later. In this setup, it is desirable to push intermediate modules to be KB-agnostic as far as possible along the pipeline.
%as that would likely result in improved generalizability, because then only a few modules later in the pipeline need to get adapted to change of KB. 
%Following that, we will describe KB-agnostic and KB-sepcific modules in detail along with the two rule modules that help reasoning extensions. 
%We use  temporal reasoning as an add on reasoning along with standard multi-hop reasoning to show how system adapts to new reasoning types through the two rule modules in the pipeline.
\begin{figure*}[t!]
  \centering
  \includegraphics[width=0.9\linewidth]{./figures/ExampleQuestion}
  %\includegraphics{./figures/pipeline}
  \caption{An illustration of the outputs at the intermediate stages of the pipeline in~\system}  
  \label{fig:example} 
\end{figure*}
\noindent
\input{text/data/lambda}
\input{text/approach/kb-agnostic}
\input{text/approach/kb-specific}

==> TempQA-AAAI2022(2)/text/approach/kb-agnostic.tex <==
\subsection{KB-Agnostic Question Understanding}
The modules in this stage aim at deriving logical expressions of the natural language question that is common for all the knowledge bases.
In particular, we use the formalism of $\lambda$-calculus for logical representation, i.e., to map questions to their corresponding $\lambda$-expressions representing the semantics.   %Each of these modules are described in the following sub-sections. 

\input{text/approach/kb-agnostic/amr}
%\input{text/approach/kb-agnostic/entity_relation_extraction}
\input{text/approach/kb-agnostic/lambda}


==> TempQA-AAAI2022(2)/text/approach/kb-agnostic/algorithm.tex <==
\begin{algorithm}[htb]
\begin{small}
%\footnotesize
 \caption{AMR to $\lambda$-expression}
 \label{alg:amrTolambda}
\SetAlgoLined
\DontPrintSemicolon
%\KwResult{Write here the result }
%\SetKwInput{KwIn}{Input}
%\SetKwInOut{Input}{Input}
%\Input{$amr$: AMR graph}
\SetKwFunction{FMain}{Convert}
\SetKwProg{Fn}{Function}{:}{}
  \Fn{\FMain{$amr\_root$}}{
        $expr = empty\_expr()$\;
        \eIf{$multi\_event(amr\_root)$}
        {
            $amr\_list$ = $break\_amr(amr\_root)$
            $connective$ = $get\_temp\_connective(amr\_root, amr\_list)$
            \For{each $amr$ in $amr\_list$}
            {
                $sub\_expr = Convert(amr)$\;
                append $sub\_expr$ to $expr$\;
            }
            append $connective$ to $expr$\;
        }
        {
            \For{each $child$ in $children(amr\_root)$}
            {
                $child\_expr = Convert(child)$\;
                append $child\_expr$ to $expr$\;
            }
            $expr = get\_expr(amr\_root, expr)$\;
            %append $e$ to $expr$\;
        }
        \KwRet $expr$\;
  }
  \end{small}
\end{algorithm}

==> TempQA-AAAI2022(2)/text/approach/kb-agnostic/amr.tex <==
\subsubsection{AMR}
%We use AMR (Abstract Meaning Representation) \cite{banarescu2013} to mediate between natural language questions and the formal query language.
In order to have a generic parse (logical expression) that is common across KBs,~\system~performs initial language understanding using Abstract Meaning Representation (AMR) \cite{banarescu2013}, a semantic representation language based on PropBank. AMR  encodes the meaning of a sentence into a rooted directed acyclic graph where nodes represent concepts and edges represent relations. %Such a representation is already an efficient step ahead in our goal of deriving $\lambda$-expressions. 
We adopt an action pointer transformer architecture of \citet{JoeZhou2021} for transition-based AMR parsing and self-training technique of \citet{YoungSuk2020} for domain adaptation to KBQA. 

AMR provides generic  representation that can be used for multi-hop reasoning~\cite{pavan2020}. However for temporal expressions with \textit{:time} relation, we have to augment the AMR annotations with implicit predicates that cannot be captured by ellipsis and/or re-entrancies. 
%Input sentence \textit{what team did michael jordan play for after baseball?} is annotated, as in Figure~\ref{fig:temporal}, which explicitly encodes the missing predicate \textit{play-01} along with its arguments ARG0, co-referred to ARG0 of \textit{play-01}, and ARG1 \textit{baseball}.
An example of AMR annotation for the question \textit{Who was US president during cold war?} is given in Figure~\ref{fig:example}. The representation encodes time edge with cold war event as sub-event of time. Also in case of before/after constraints it explicitly captures the constraint as part of the time edge.
If there are no explicit constraints like before/after or ordinal in the time edge, we treat them as overlap constraints. %More details on how different AMR frames are converted to appropriate $\lambda$ expressions.
%It encodes the missing predicate \textit{play-01} along with its argument ARG0, co-referred to the ARG0 of the top concept \textit{play-01}. 
%Note that the temporal phrase \textit{time} is treated like \textit{before he played for man city} to capture the intended meaning.
%\begin{figure}
%\begin{verbnobox}[\fontsize{8pt}{8pt}\selectfont]
%(p / play-01
%   :ARG0 (p2 / person 
%            :name (n / name 
%                    :op1 "Michael" 
%                    :op2 "Jordan"))
%   :beneficiary (t / team
%                   :mod (a / amr-unknown))
%   :time (a2 / after
%            :op1 (p3 / play-01
%                  :ARG0 p2
%                  :ARG1 (b / baseball))))
%\end{verbnobox}
%\caption{AMR annotations for \textit{what team did michael jordan play for after baseball?}. The %temporal phrase \textit{after baseball} is paraphrased as \textit{after he played baseball} to capture %the intended semantics.}
%\label{fig:temporal}
%\end{figure}
%AMR parser performances on the development testsets are shown in Table~\ref{tab:amr_performance}. 

%\begin{table}[htb]
%\begin{small}
%\centering
%\setlength\tabcolsep{6pt}
%\renewcommand{\arraystretch}{1.0}
%\begin{tabular}{lcc}
%\toprule
%\multirow{2}*{Dataset}   & %\multicolumn{2}{c}{Accuracy}  \\
%& Smatch  & Exact Match \\
%\midrule
%TempQA-WD & $89.6$  & $40.2$ \\
%SWQ-WD & $82.9$ &  $38.3$\\
%WebQSP-WD & $88.0$ & $46.3$ \\
%\bottomrule
%\end{tabular}
%\caption{AMR parser performance on %development sets. Exact Match indicates %the ratio of perfect parses.}
%\label{tab:amr_performance}
%\end{small}
%\end{table}



==> TempQA-AAAI2022(2)/text/approach/kb-agnostic/entity_relation_extraction.tex <==
\subsubsection{Entity and Relation Extraction:}
\label{sec:entity-rel-ext}
%The goal here is to spot mentions of entities and relations in the question. 
We use AMR mentions as entity mentions and Propbank frames as relation mentions.
%We extract those directly from the AMR as they are already encoded in AMR as nodes and edges.
%Our system make use of AMR to detect entities and relationships of questions. 
%AMR marks entity surface forms detected in the question text as sink nodes in the AMR graph with quotes mark. Relationships are captured by %Proposition Bank or 
%PropBank Frames AMR nodes. PropBank frame nodes denotes relationship between its children node. %In relationship detection, 
We handle all cases of PropBank frame nodes with arity less than 3 and partially handle 3 or more arity cases. %However, we have observed that there are small number of instances where PropBank node falls in unhandled category. But we'll generalize it and work on these cases in future.

==> TempQA-AAAI2022(2)/text/approach/kb-agnostic/lambda.tex <==
\subsubsection{KB-Agnostic Lambda Expression}
AMR is a fairly granular representation. However, for a KBQA system, specifically on KGs such as DBpedia, Wikidata, and Freebase, such granularity can add noise. Therefore to construct KB-agnostic  $\lambda$-expressions of the questions from their corresponding AMRs and their identified entity and relation mentions, we use the transformational heuristics described in  Table~\ref{tab:amrTranslation}. 
%As described in Section \ref{sec:lambda} and also as illustrated in Figure~\ref{fig:example} for an example question, $\lambda$-expressions represent semantics of the questions in a logical form, specifically as a conjunction of sub-expressions. 
%In $\lambda$-expression, temporal events, corresponding time intervals and the temporal reasoning are also captured as sub-expressions.
%This KB-agnostic representation of the question semantics as a $\lambda$-expression also provides an effective base work to map onto KB-specific expressions later in the pipeline.
The table shows the transformation from AMR frame (high level) to the corresponding Lambda expression. The rule type describes where the rule is in general applied to all reasoning (base) vs temporal. 
%etc, and second column gives the high level structure of the AMR frame and the third column describes the corresponding structure of Lambda expression that will get generated. Base rules and numerical rules in this table cover most of the existing KBQA datasets. 
We handle these as conjunction of multiple triples in the KB with some projection variable and/or numerical operation to get the final answer. We use AMR unknown/imperative constructs to identify the projection variables and AMR polarity/interrogative frames for queries which fall into boolean answers or ASK questions in SPARQL. 
% Figure \ref{fig:example} shows an example of AMR to Lambda conversion process using our running example. 
% A simple example for AMR to Lambda conversion process using base rules is shown
% in Figure~\ref{fig:singlehopExample}. %\mdc{What happens when there's no ARG0?}
% Note that $\lambda$-expression has different entity mention as opposed to AMR in the example. We use a BERT based named entity detection module trained using multiple KBQA datasets. We use mentions coming from this module to align and collapse the AMR nodes to capture known KB mentions. In this question \emph{Ford Y - Block Engine} is a mention that is used to collapse node e in AMR and is used as an entity mention in the generated Lambda expression.

The next set of rules present in Table~\ref{tab:amrTranslation} are few sample template rules used to capture temporal events and constraints to help in temporal reasoning.  Figure~\ref{fig:example} gives an example question that falls into the temporal overlap rule in the table and how the AMR constructs are used to split the events is highlighted with nodes being bold in the table. Complete set of rules used can be found in the supplementary material. Note that we covered temporal reasoning as an additional form of reasoning in the current system. However,  more reasoning templates like spatial reasoning with additional operators like \textit{coordinates(), south()} ...etc can be added. Table~\ref{tab:amrTranslation} shows an example template for spatial questions such as \textit{"which states are to the south of California?"}.
% \begin{figure}[th]
%   \centering
%   \includegraphics[height=4cm, width=7cm]{./figures/SingleHopExample}
%   \vspace{-0.35cm}
%   \caption{Example for AMR to Lambda conversion}
%   \label{fig:singlehopExample} 
% \end{figure}

%Algorithm~\ref{alg:amrTolambda} shows AMR to $\lambda$-expression conversion process. 
%This algorithm contains a recursive function $Convert()$ that takes AMR $root\_node$ as its input. Within this, function $multi\_event()$ is used to handle single event vs multiple events (two or more events) in two distinct blocks. In case of multiple events, AMR is divided into multiple component AMRs using function $break\_amr()$ and each of those are converted to $\lambda$-expressions individually, and then combined together using appropriate $connective$ \textit{(overlap, before, after)}. In case of single event, it is converted by recursively processing of each child of $amr\_root$. After processing each child, $\lambda$-expressions of all children are combined by adding them together to get the $\lambda$-expression of the $amr\_root$.

%In our system we use Lambda Expression, inspired by $\lambda$-calculus, to logically represent the question. Originally $\lambda$-calculus was an effort to formalise functions as a means of computing, but recently it has been used for semantic parsing in natural language question answering systems. With $\lambda$-expression we capture the logical form of natural language question by comprising entities and relationships. These entities and relationships are mapped to KB entities and relationships in later stages.

%As explained earlier, we rely on AMR to construct $\lambda$-expression for question text. AMR is DAG in nature and it has no relationship with any Knowledge base. With our system, we aim use RDF Knowledge Base (such as Wikidata and DBpedia) to get answer, where data is stored in triple form. For this reason, AMR is converted into $\lambda$-expression such that each of its sub-expression follow triple pattern. For instance, $\lambda$-expression, shown in Figure~\ref{fig:example}, has sub-expression $play$-$01(e_1, ``Joe\ Hart", t)$ which represents $play$ relationship between ${Joe\ Hart}$ and variable $t$.

%In addition, other motive of $\lambda$-expression is to capture different temporal events from question through AMR. We use \textit{:time} AMR edge to find temporal events. Thereafter, temporal quantifies, introduced in Section~\ref{sec:lambda}, are utilized to associate time with events (using \textit{interval}) and apply temporal reasoning (using \textit{overlap, before, after}).


%Further, AMR to $\lambda$-expression conversion is explained using Algorithm~\ref{alg:amrTolambda}. It presents high level logic behind the conversion process. This algorithm contains a recursive function $Convert()$ which takes AMR $root\_node$ as argument. This function mainly has two blocks, first when AMR has more then two events, second if AMR consists single event only. This condition is checked with function $multi\_event()$. In case of mutiple events, AMR is divided into multiple AMRs using function $break\_amr()$ then those AMRs are converted to $\lambda$-expressions individually. These individual $\lambda$-expressions are combined along with appropriate $connective$ \textit{(overlap, before, after)}.

%If AMR has single event only, it is converted by recursively processing each child of $amr\_root$. After processing each child, their $\lambda$-expression is combined with adding $\lambda$-expression of $amr\_root$.

% In our system we also use it for logical representation of questions. As an example, consider the question text and corresponding logical form:

% \begin{center}
% \begin{tabular}{l l}
%  Question: & Where did Barac Obama born\\ 
%  Logical Form: & $\lambda$l. born(``Barac Obama", l)\\  
% \end{tabular}
% \end{center}

% In our system, we rely on AMR to construct lambda expression for question text. As AMR contains high level abstract representation of text, we make use of it to generated intermediate logical representation. It mainly comprises entity and their relations in structured form. In addition, as temporal system, we use AMR to identify temporal events and their relation also.

% Lambda expression contains constant to denote entities, functions, numbers, date etc. Lambda variables are used to denote unknowns. Further, it uses logical connectives to connect subexpressions. We also make use of additional quantifiers such as \textit{min, max, argmax, argmin} etc. for advance operations. We have introduced temporal functions for handling temporal reasoning. It includes \textit{interval(), overlap(), before(), after()} etc.

% \textbf{AMR to Lambda Expression}: For obtaining Lambda, following steps are followed: \begin{itemize}
%   \item Events are identified using AMR.
%   \item For each event, its AMR graph is recursively transformed into Lambda expression. 
%   \item For each temporal event time expression is added and temporal connective condition added based on temporal signal present in AMR. 
% \end{itemize} 


\begin{table*}[htb] \setlength\tabcolsep{7pt}
    \centering
    \begin{small}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{lll}%{@{}l{} @{~~~} l{} @{~~~} l{}@{}} 
    
        \toprule
        \begin{tabular}[l]{@{}l@{}}
           \textbf{Rule}\\
           \textbf{Type}
        \end{tabular} 
        &
        \textbf{AMR A = (v/frame …)}
        &
        \textbf{Lambda Expression L = $\psi$(v)} 
        \\ 
        \midrule
        
        
        \begin{tabular}[l]{@{}l@{}}
           Base
        \end{tabular} 
         &
         \begin{tabular}[l]{@{}l@{}}
            (\textbf{v}/frame :arg0(\textbf{v0}/frame0) … :argn(\textbf{vn}/framen))
        \end{tabular} 
         &
         \begin{tabular}[c]{@{}l@{}}
            frame(\textbf{v}, \textbf{v0}, … \textbf{vn}) $\land$ $\psi$(\textbf{v0}) $\land$ … $\psi$(\textbf{vn}) 
        \end{tabular} 
        \\
         \noalign{\smallskip}
         
         
         \begin{tabular}[l]{@{}l@{}}
           Base
        \end{tabular} 
         &
         \begin{tabular}[l]{@{}l@{}}
            (\textbf{v}/frame :\textbf{arg1(a/amr-unknown)}  … :argn(vn/framen))
        \end{tabular} 
         &
         \begin{tabular}[c]{@{}l@{}}
           $\lambda$a. $\psi$(\textbf{v})
        \end{tabular} 
        \\
         \noalign{\smallskip}
        
        
    %      \begin{tabular}[l]{@{}l@{}}
    %       Numerical
    %     \end{tabular} 
    %      &
    %      \begin{tabular}[l]{@{}l@{}}
    %         (v/frame :arg0(v0/frame0) … :argn(vn/framen :arg1-of\\ (h2/\textbf{have-degree-91} :arg3(m/\textbf{more}) :arg4(vm/framem\\ :arg1-of(n/nested-frame))))
    %     \end{tabular} 
    %      &
    %      \begin{tabular}[c]{@{}l@{}}
    %          $\psi$(v) $\land$ $\psi$(n) $\land$ cmp(vn, vm, $>$) 
    %     \end{tabular} 
    %     \\
    %      \noalign{\smallskip}
         
         
    %   \begin{tabular}[l]{@{}l@{}}
    %       Numerical
    %     \end{tabular} 
    %      &
    %      \begin{tabular}[l]{@{}l@{}}
    %         (v/frame :arg0(v1/frame1:mod(a/amr-unknown)) …:argn\\
    %         (vn/frame :arg1-of(h2/\textbf{have-quant-91} :arg3(l/\textbf{most}))))

    %     \end{tabular} 
    %      &
    %      \begin{tabular}[c]{@{}l@{}}
    %          argmax($\lambda$v1. $\psi$(v1), $\lambda$v1. $\lambda$vn. $\psi$(v), 0, 1)
    %     \end{tabular} 
    %     \\
    %      \noalign{\smallskip}
         
         \begin{tabular}[l]{@{}l@{}}
           Numerical
        \end{tabular} 
         &
         \begin{tabular}[l]{@{}l@{}}
            (\textbf{v}/frame :arg0(\textbf{v0}/frame0 :\textbf{quant(a/amr-unknown})) …\\ :argn(vn/framen))
        \end{tabular} 
         &
         \begin{tabular}[c]{@{}l@{}}
            count($\lambda$\textbf{v0}. $\psi$(\textbf{v}))
        \end{tabular} 
        \\
         \noalign{\smallskip}
         
         
        
         \begin{tabular}[l]{@{}l@{}}
          Temporal
        \end{tabular} 
         &
         \begin{tabular}[l]{@{}l@{}}
            (\textbf{v}/frame :arg0(v0/frame0) … :argn(vn/framen)\\
            \textbf{:time(a/amr-unknown))}
        \end{tabular} 
         &
         \begin{tabular}[c]{@{}l@{}}
          $\lambda$ev. $\psi$(\textbf{v}) $\land$ interval(ev, \textbf{v}) 
        \end{tabular} 
        \\
         \noalign{\smallskip}
         
         
        \begin{tabular}[l]{@{}l@{}}
           Temporal
        \end{tabular} 
         &
         \begin{tabular}[l]{@{}l@{}}
            (\textbf{v}/frame :arg0(a/amr-unknown) … :argn(vn/framen)\\
            \textbf{:time(b/before} :op1(\textbf{n}/nested-frame)))
        \end{tabular} 
         &
         \begin{tabular}[c]{@{}l@{}}
           argmax($\lambda$a. $\psi$(\textbf{v}) , $\lambda$a. $\lambda$ev. $\psi$(\textbf{n}) $\land$ interval(ev, \textbf{v}) \\
           $\land$ interval(en, \textbf{n}) $\land$ \textbf{before}(ev, en), 0, 1)
        \end{tabular} 
        \\
         \noalign{\smallskip}
         
         
        %  \begin{tabular}[l]{@{}l@{}}
        %   Temporal
        % \end{tabular} 
        %  &
        %  \begin{tabular}[l]{@{}l@{}}
        %     (v/frame :arg0(a/amr-unknown) … :argn(vn/framen)\\
        %     \textbf{:time(a/after} :op1(n/nested-frame)))
        % \end{tabular} 
        %  &
        %  \begin{tabular}[c]{@{}l@{}}
        %   argmin($\lambda$a. $\psi$(v) , $\lambda$a. $\lambda$ev. $\psi$(n) $\land$ interval(ev, v) \\
        %   $\land$ interval(en, n) $\land$ \textbf{after}(ev, en), 0, 1)
        % \end{tabular} 
        % \\
        %  \noalign{\smallskip}
         
         
        \begin{tabular}[l]{@{}l@{}}
           Temporal
        \end{tabular} 
         &
         \begin{tabular}[l]{@{}l@{}}
            (\textbf{v}/frame :arg0(a/amr-unknown) … :argn(vn/framen)\\
            \textbf{:time}(\textbf{n}/nested-frame))
        \end{tabular} 
         &
         \begin{tabular}[c]{@{}l@{}}
           $\lambda$a. $\psi$(\textbf{v}) $\land$ $\psi$(\textbf{n}) $\land$ interval(ev, \textbf{v}) $\land$ interval(en, \textbf{n})\\
           $\land$ \textbf{overlap}(ev, en)
        \end{tabular} 
        \\
         \noalign{\smallskip}
         
         
        % \begin{tabular}[l]{@{}l@{}}
        %   Temporal
        % \end{tabular} 
        %  &
        %  \begin{tabular}[l]{@{}l@{}}
        %     (v/frame :arg0(a/amr-unknown) … :argn(vn/framen)\\
        %     \textbf{:time(n/now))}
        % \end{tabular} 
        %  &
        %  \begin{tabular}[c]{@{}l@{}}
        %   $\lambda$a. $\psi$(v) $\land$ interval(ev, v) $\land$ interval(en, now()) \\
        %     $\land$ overlap(ev, en)
        % \end{tabular} 
        % \\
        %  \noalign{\smallskip}
         
         
        % \begin{tabular}[l]{@{}l@{}}
        %   Temporal
        % \end{tabular} 
        %  &
        %  \begin{tabular}[l]{@{}l@{}}
        %     (v/frame :arg0(a/amr-unknown) … :argn(vn/framen)\\
        %     \textbf{:time(d/date-entity} :month mm :day dd :year yyyy))
        % \end{tabular} 
        %  &
        %  \begin{tabular}[c]{@{}l@{}}
        %   $\lambda$a. $\psi$(v) $\land$ interval(en, date(“dd-mm-yyyy”)) \\ $\land$ interval(ev, v) $\land$ overlap(ev, en)
        % \end{tabular} 
        % \\
        %  \noalign{\smallskip}
     
        
        %  \begin{tabular}[l]{@{}l@{}}
        %   Temporal
        % \end{tabular} 
        %  &
        %  \begin{tabular}[l]{@{}l@{}}
        %     (v/frame :arg0(a/amr-unknown) … :argn(vn/framen)\\
        %     \textbf{:time(t/teenager} :domain(n/nested-frame)))
        % \end{tabular} 
        %  &
        %  \begin{tabular}[c]{@{}l@{}}
        %   $\lambda$a. $\psi$(v) $\land$ $\psi$(n) $\land$ interval(ev, v) $\land$ teenager(en, n) \\
        %   $\land$ overlap(ev, en)
        % \end{tabular} 
        % \\
        %  \noalign{\smallskip}
     
         \begin{tabular}[l]{@{}l@{}}
           Spatial
        \end{tabular} 
         &
         \begin{tabular}[l]{@{}l@{}}
            (\textbf{b}/\textbf{be-located-at-91} :arg0(a/amr-unknown),\\ \textbf{:mod(s/south)} :op1(\textbf{n}/nested-frame))
        \end{tabular} 
         &
         \begin{tabular}[c]{@{}l@{}}
           $\lambda$a. $\psi$(\textbf{b})$\land$  $\psi$(\textbf{n}) $\land$ coordinate(cb, \textbf{b}) $\land$ coordinate(cn, \textbf{n})\\
           $\land$ \textbf{south}(cb, cn)
        \end{tabular} 
        \\
         \noalign{\smallskip}
         
         
    \bottomrule
    \end{tabular}
    }
    \end{small}
    \caption{AMR to Lambda Translation}
    \label{tab:amrTranslation}
\end{table*}



==> TempQA-AAAI2022(2)/text/approach/kb-specific.tex <==
\subsection{Question Mapping and Reasoning}
This is the second stage which comprises of modules that transform the KB-agnostic $\lambda$-expression of the questions into KB-specific $\lambda$-expression. These modules are entity linking and relationship linking that are specific to the underlying KB along with any KB specific rules to handle special forms of transformation or reasoning. The modules are interchangeable to different knowledge graphs. Currently, we demonstrate the adaptability of these modules to DBpedia and Wikidata. 

%that when executed over the KB would derive the answer. Each of these modules are descried in the following sub-sections.
\input{text/approach/kb-specific/kb_lambda}
\input{text/approach/kb-specific/entity_linking}
\input{text/approach/kb-specific/relation_linking}
\input{text/approach/kb-specific/sparql}


==> TempQA-AAAI2022(2)/text/approach/kb-specific/entity_linking.tex <==

\noindent\textbf{\emph{Entity Linking:}} The goal of Entity Linking is to map entity mentions as captured in the $\lambda$-expression of the question to their corresponding KB-specific entities. We use a recently proposed zero-shot entity linking approach called BLINK \cite{BLINK}. For a question where entity mentions are already identified, bi-encoder piece of the BLINK is used to predict top-K entities. For this prediction, we use an entity dictionary of 5.9M English Wikipedia entities, mapped to their corresponding Wikidata  and DBpedia entities. 
%We used the 100\% bi-encoder model of BLINK for all the datasets used in our experiments.
%on 5\% Wikipedia training data released by the authors of BLINK, as that resulted in improved performance in shorter training time. 
%Table~\ref{EL_performance} shows our entity linking performance on two different datasets. Question level accuracy is computed by taking into account all the entities in the question, while mention level accuracy is computed on individual mentions.

%A closer look into the results show that accuracy on nominal entities (which BLINK is not trained on) drags down the question level accuracy on TempQA dataset. For SWQ dataset, the question size becomes bottleneck as that leads to lack of adequate context. Also some of the SWQ entities are not present in the entity dictionary.

%For the purpose of entity linking (i.e. disambiguation), we use a recently proposed zero-shot entity linking approach  called BLINK~\cite{BLINK}. We use only bi-encoder piece of the BLINK and predict top-$k$ entities for any given input question where entity mention has already been identified. The set of predicted entities comes from a corpus of $5.9$M English Wikipedia entities which are then mapped to their corresponding Wikidata Q-id. We retrained the bi-encoder model of BLINK on Wikipedia training set released by the authors of BLINK~\cite{BLINK} paper. For this training, we used only 5\% of the original training data as it offered slightly better performance and also the training time was much less.  Table \ref{EL_performance} below captures the performance of our entity linking task on gold mentions of entities from two different datasets. The question level accuracy is computed by considering all the entities present in each question. However, mention level accuracy is computed by considering single mention at a time.
%-------------------------------------------
%\begin{table}[htb]
%\begin{small}
%\centering
%\setlength\tabcolsep{6pt}
%\renewcommand{\arraystretch}{1.0}
%\begin{tabular}{lrr}
%\toprule
%\multirow{2}*{Dataset}   & %\multicolumn{2}{c}{Accuracy (\%)}  \\
%& Mention Level & Question Level \\
%\midrule
%TempQA-WD & $69.71$  & $48.93$ \\
%SWQ-WD & $70.00$ &  $67.70$\\
%\bottomrule
%\end{tabular}
%\caption{Entity linking performance on %development sets when gold mentions are %provided.}
%\label{EL_performance}
%\end{small}
%\end{table}
%------------------------------------------- 
%The question level performance on TempQA dataset is low due to the presence of nominal entities (e.g. “city”, “film”) for which BLINK is not trained on. BLINK is mostly trained on the named-entities. Training BLINK to handle nominal entities is a future direction for us. Similarly, for SWQ dataset, the performance bottleneck include factors such as {\em very short question text} and because of which there is not adequate context available to disambiguate entities. Also, in SWQ dataset, some of the gold entities (based on Wikidata) are absent from English Wikipedia and hence from our corpus as well. 

==> TempQA-AAAI2022(2)/text/approach/kb-specific/kb_lambda.tex <==
\subsubsection{KB-Specific Lambda Expression:}
%This part of pipeline makes use of entity linking and relation linking to map $\lambda$-expression entities and relations to knowledge base entities and relations and generate KB-Specific $\lambda$-expression. 
Structurally, it is similar to $\lambda$-expression with all entities and relations mapped to KB entities and relations respectively. 
%This module is also responsible for finding additional \textit{Wikidata} temporal relations for events in order to extract their associated time intervals. 
%This involves checking the existence and fetching reified relation. If refied relation is absent, simple time relation is identified.


==> TempQA-AAAI2022(2)/text/approach/kb-specific/relation_linking.tex <==
\noindent\textbf{\emph{Relation Linking:}}
%Our system uses a relation linking component that
\system's Relation linking component
takes in the question text and an AMR graph as input and returns a ranked list of KG relationships. For instance, given a question such as "Who was the US President during cold war?" (see Fig~\ref{fig:example}) and the corresponding AMR, the goal of the relation linking component is to find the corresponding Wikidata KB relations \textit{position held (P39)}, \textit{start time (P580)}, \textit{end time (P582)}. For this task, we use state-of-the-art AMR-based relation linking approach with models built for both DBpedia and Wikidata~\cite{naseem-etal-2021-semantics}.

%The Relation Linking component is driven by $\lambda$-expressions of the questions extracted from the question. The main neural relation prediction module is modelled as a Siamese network, where the input question and target relations are embedded in the same vector space and the most likely relation is predicted based on the closeness of its representation with that of the input question.  It use a Transformer model~\cite{vaswani2017attention} as a shared encoder for both the input questions and candidate relations and uses a pre-trained BERT model~\cite{devlin2018bert} to initialize the encoder parameters. 
%The output vector corresponding to the starting \textsc{[CLS]} token is used as the vector representation of the input. This vector is passed through a feed-forward linear layer that projects it to the shared embedding space. 
%We used  LC-QuAD 2.0~\cite{lcquad2} dataset to train this model for predicting Wikidata relations.

%Table~\ref{RL_performance} shows the performance of relation linking component on the dev set mentioned in Section~\ref{sec.dataset_details}.

%-------------------------------------------
%\begin{table}[h]
%\centering
%\setlength\tabcolsep{6pt}
%\renewcommand{\arraystretch}{1.0}
%\begin{tabular}{lrrr}
%\toprule
%{Dataset} & P & R & F1 \\
%\midrule
%TempQA & $xx.xx$  & $xx.xx$ & $xx.xx$ \\
%SWQ & $xx.xx$ &  $xx.xx$ & $xx.xx$ \\
%\bottomrule
%\end{tabular}
%\caption{Relation linking performance on development sets when gold entities are provided.}
%\label{RL_performance}
%\end{table}
%------------------------------------------- 

==> TempQA-AAAI2022(2)/text/approach/kb-specific/sparql.tex <==
\noindent\textbf{\textit{{SPARQL Query:}}}
This module maps KB-specific  $\lambda$-expressions onto SPARQL queries through a deterministic approach. Each KB-specific $\lambda$-expression construct is mapped to an equivalent SPARQL construct, as rules given in Table~\ref{tab:kbSpecificTranslation}.
% $\lambda$-expressions in our setup can be broadly grouped into 5 categories: \textit{$\lambda$ abstraction}, \textit{argmin}, \textit{argmax}, \textit{min}, and \textit{max} expression. Table \ref{tab:kbSpecificTranslation} gives mapping for \textit{$\lambda$ abstraction}, \textit{argmin}, and \textit{min}. Mappings for \textit{argmax} and \textit{max} are similar to that of \textit{argmin} and \textit{min} respectively, except the direction of ORDER BY is changed to DESC.
Each of lambda expressions contains one or more terms such that each term $T_i$ is comprised of one or more predicates connected via $\land$ or $\lor$. Translation of different predicates is present in Table~\ref{tab:kbSpecificTranslation}. Some of the KB-spe cific aspects like handling reification in Wikidata are shown in the Table.
To get the time interval in case of reified events, \textit{Start time(wdt:P580)}, \textit{end time(wdt:P582)}, or \textit{point in time(wdt:P585)} connected to intermediate statement node are used. 
%Sub-expressions that appear in $\lambda$-expressions are broadly of types \textit{Wikidata} predicate, \textit{interval}, and \textit{temporal} functions. \textit{Wikidata} predicate is directly mapped to triple patterns in SPARQL, whereas \textit{interval} creates time intervals consisting of start time and end time for the corresponding event. To construct time intervals in case of reified events \textit{Start time(wdt:P580)}, \textit{end time(wdt:P582)}, or \textit{point in time(wdt:P585)} information as present in the reified fields are used, whereas for non-reified events other temporal properties associated with the entity are used. \textit{Teenager} function uses \textit{date of birth(wdt:P569)} to get time interval, while \textit{now} event uses \textit{current time(now())}. Temporal functions such as \textit{overlap}, \textit{before}, and \textit{after} make use of FILTER condition to filter out those intervals that do not satisfy the corresponding conditions.
%This module transforms KB-specific lambda expression into a SPARQL query. The deterministic approach described in Table \ref{tab:kbSpecificTranslation} is used for achieving this transformation where each construct present in KB specific lambda is mapped to an equivalent SPARQL construct. 
%Lambda expression used in the proposed approach can be broadly categorized into 5 categories: \textit{lambda abstraction}, \textit{argmin}, \textit{argmax}, \textit{min}, and \textit{max} expression. Mapping for \textit{lambda abstraction}, \textit{argmin}, and \textit{min} expression is presented in Table \ref{tab:kbSpecificTranslation}. \textit{argmax} and \textit{max} follow an approach similar to \textit{argmin} and \textit{min} respectively with the direction of ORDER BY changed to DESC. Each of these expressions might contain one or more terms such that each term $T_i$ comprises of one or more predicates connected via $\land$ or $\lor$. 
%Predicates used in lambda expression can be broadly categorized into \textit{wikiData predicate}, \textit{interval} predicate, and temporal predicate. WikiData predicate is directly mapped to triple pattern in SPARQL, whereas the Interval predicates create an interval consisting of start time and end time for a given event. \textit{Start time(wdt:P580)}, \textit{end time(wdt:P582)}, or \textit{point in time(wdt:P585)} present in case of reified events can be used for creating the interval, whereas for non-reified events a temporal property associated with the entity is used to construct the interval. \textit{Teenager} predicate and \textit{now} make use of \textit{date of birth(wdt:P569)} and \textit{current time(now())} respectively for creating the interval. Temporal predicates include \textit{overlap}, \textit{before}, and \textit{after} which make use of FILTER condition to filter out the intervals that did not follow the specific conditions. 

\begin{table*}[htb] \setlength\tabcolsep{7pt}
    \centering
    % \scriptsize
    \begin{small}
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{lll} %{@{}l{} @{~~~} l{} @{~~~} l{}@{}} 
        \toprule
        \textbf{Type} &\textbf{ Expression/Predicate E} & \textbf{SPARQL S = $\phi$(E)} \\ 
        \midrule
        
        \begin{tabular}[l]{@{}l@{}}
            $\lambda$ abstraction
        \end{tabular} 
         &
         \begin{tabular}[l]{@{}l@{}}
            $\lambda$x.T
        \end{tabular} 
         &
         \begin{tabular}[c]{@{}l@{}}
          SELECT DISTINCT ?x WHERE \{ $\phi$(T) \}
        \end{tabular} 
        \\
         \noalign{\smallskip}
        
        
        \begin{tabular}[l]{@{}l@{}}
          Count expression
        \end{tabular} 
         &
        \begin{tabular}[l]{@{}l@{}}
             count($\lambda$x.T)
        \end{tabular} 
         &
         \begin{tabular}[c]{@{}l@{}}
          SELECT (COUNT(?x) AS ?c) WHERE \{ $\phi$(T) 
          \}
        \end{tabular}
        \\
         \noalign{\smallskip}
        
        
        % \begin{tabular}[l]{@{}l@{}}
        %   Argmin expression
        % \end{tabular} 
        %  &
        % \begin{tabular}[l]{@{}l@{}}
        %      argmin($\lambda$x.T$_1$, $\lambda$x.$\lambda$y.T$_2$,\\ off, lim)
        % \end{tabular} 
        %  &
        %  \begin{tabular}[c]{@{}l@{}}
        %   SELECT DISTINCT ?x WHERE \{ $\phi$(T$_1$) $\phi$(T$_2$) \\
        %   \} ORDER BY (?yStart) LIMIT lim OFFSET off
        % \end{tabular}
        % \\
        %  \noalign{\smallskip}
        
        
        
        \begin{tabular}[l]{@{}l@{}}
          Argmax expression
        \end{tabular} 
         &
        \begin{tabular}[l]{@{}l@{}}
             argmax($\lambda$x.T1, $\lambda$x.$\lambda$y. T2, \textit{O}, \textit{L})
        \end{tabular} 
         &
         \begin{tabular}[c]{@{}l@{}}
          SELECT DISTINCT ?x WHERE \{
           $\phi$(T1)  $\phi$(T2) \\
          \} ORDER BY DESC(?yStart) LIMIT \textit{L} OFFSET \textit{O}
        \end{tabular}
        \\\noalign{\smallskip}
        %  \begin{tabular}[l]{@{}l@{}}
        %   Min expression
        % \end{tabular} 
        %  &
        % \begin{tabular}[l]{@{}l@{}}
        %      min($\lambda$x.T, off, lim)
        % \end{tabular} 
        %  &
        %  \begin{tabular}[c]{@{}l@{}}
        %   SELECT DISTINCT ?x WHERE \{ $\phi$(T) \\
        %   \} ORDER BY (?xStart) LIMIT lim OFFSET off
        % \end{tabular}
        % \\
        %  \noalign{\smallskip}
        
        
        
        %  \begin{tabular}[l]{@{}l@{}}
        %   Max expression
        % \end{tabular} 
        %  &
        % \begin{tabular}[l]{@{}l@{}}
        %      max($\lambda$x.T, o, l)
        % \end{tabular} 
        %  &
        %  \begin{tabular}[c]{@{}l@{}}
        %   SELECT DISTINCT ?x WHERE \{\\
        %   \tab $\phi$(T) \\
        %   \} ORDER BY DESC(?xStart) LIMIT l OFFSET o
        % \end{tabular}
        % \\\noalign{\smallskip}
        
        
        
        \begin{tabular}[l]{@{}l@{}}
          KB Predicate
        \end{tabular} 
         &
        \begin{tabular}[l]{@{}l@{}}
            IRI$_p$(r, s$|$IRI$_s$, o$|$IRI$_o$)
        \end{tabular} 
         &
         \begin{tabular}[c]{@{}l@{}}
          ?s$|$IRI$_s$ IRI$_p$ ?o$|$IRI$_o$.
        \end{tabular} 
        \\
         \noalign{\smallskip}
        
        
        
        \begin{tabular}[l]{@{}l@{}}
            Interval predicate\\ for reified facts
        \end{tabular} 
         &
        \begin{tabular}[l]{@{}l@{}}
             wdt:PID(e, s$|$wd:QID$_1$, o$|$wd:QID$_2$)\\
             $\land$ interval(e$^i$, e)
        \end{tabular} 
         &
         \begin{tabular}[c]{@{}l@{}}
          ?s$|$wd:QID$_1$ p:PID ?e. ?e ps:PID ?o$|$wd:QID$_2$.\\
          ?e \textit{pq:P580} ?eiStart. ?e \textit{pq:P582} ?eiEnd.
        \end{tabular} 
        \\
         \noalign{\smallskip}
    
    
        % \begin{tabular}[l]{@{}l@{}}
        %     Interval predicate \\for non-reified facts
        % \end{tabular} 
        %  &
        % \begin{tabular}[l]{@{}l@{}}
        %      wdt:PID(e, s$|$wd:QID, x)$\land$\\
        %      interval(e$^i$, x)
        % \end{tabular} 
        %  &
        %  \begin{tabular}[c]{@{}l@{}}
        %   ?s$|$wd:QID wdt:PID ?x.\\
        %   BIND (?x AS ?eiStart) BIND (?x AS ?eiEnd)
        % \end{tabular} 
        % \\
        %  \noalign{\smallskip}
        
        
        % \begin{tabular}[l]{@{}l@{}}
        %      Now predicate
        % \end{tabular} 
        %  &
        % \begin{tabular}[l]{@{}l@{}}
        %      now(e$^i$)
        % \end{tabular} 
        %  &
        %  \begin{tabular}[c]{@{}l@{}}
        %   BIND (now() AS ?eiStart) BIND (now() AS ?eiEnd)
        % \end{tabular} 
        % \\
        %  \noalign{\smallskip}
        
        
        
        % \begin{tabular}[l]{@{}l@{}}
        %     Teenager predicate
        % \end{tabular} 
        %  &
        % \begin{tabular}[l]{@{}l@{}}
        %     teenager(e$^i$, s$|$wd:QID)
        % \end{tabular} 
        %  &
        %  \begin{tabular}[c]{@{}l@{}}
        %   ?s$|$wd:QID wdt:P569 ?e.
        %   BIND (?e + "P13Y"$^\wedge^\wedge$xsd:duration\\ AS ?eiStart)
        %   BIND (?e + "P19Y"$^\wedge^\wedge$xsd:duration AS ?eiEnd)
        % \end{tabular} 
        % \\
        %  \noalign{\smallskip}
        
        
        \begin{tabular}[l]{@{}l@{}}
          Overlap predicate
        \end{tabular} 
         &
        \begin{tabular}[l]{@{}l@{}}
             overlap(e1$^i$ e2$^i$)
        \end{tabular} 
         &
         \begin{tabular}[c]{@{}l@{}}
          FILTER(?e1iStart<=?e2iEnd \&\&
          ?e2iStart<=?e1iEnd)
        \end{tabular} 
        \\
         \noalign{\smallskip}
        
        
        
        \begin{tabular}[l]{@{}l@{}}
            Before predicate
        \end{tabular} 
         &
         \begin{tabular}[l]{@{}l@{}}
             before(e1$^i$, e2$^i$)
        \end{tabular} 
         &
         \begin{tabular}[c]{@{}l@{}}
          FILTER(?e1iEnd<=?e2iStart)
        \end{tabular}
        \\
        \noalign{\smallskip}
        
        
        \begin{tabular}[l]{@{}l@{}}
             After predicate
        \end{tabular} 
         &
        \begin{tabular}[l]{@{}l@{}}
             after(e1$^i$, e2$^i$)
        \end{tabular} 
         &
         \begin{tabular}[c]{@{}l@{}}
          FILTER(?e1iStart>=?e2iEnd)
        \end{tabular}
        \\
        \noalign{\smallskip}
    \bottomrule
    \end{tabular}
    }
    \end{small}
    \caption{Translation of KB Specific Lambda Expression}
    \label{tab:kbSpecificTranslation}
\end{table*}

%For non-reified events other temporal properties associated with the entities in the triple are used to get the temporal information.


==> TempQA-AAAI2022(2)/text/conclude.tex <==

\section{Conclusion}

In this paper, we present \system~system that is generalizable across knowledge bases and reasoning types. We introduce KB-agnostic question understanding component that is common across KBs with AMR based intermediate $\lambda$-Calculus representation. Question Mapping and reasoning module on the specific KB is customized per KB. we also presented rule modules that can aid in adding new reasoning type. 
%In both the modules we have templated Rules that are fed to the system to drive the new reasoning type additions and illustrated it with temporal reasoning. 
We introduced a new benchmark dataset \dataset~for temporal KBQA on \textit{Wikidata}. %Adapted from existing \textit{TempQuestions} dataset, this dataset has parallel answer annotations on two KBs.  
%A subset of this dataset is also annotated with output expected at intermediate stages of the system pipeline. 
Experimental results show that \system ~indeed achieves its generalization goals with state of the art results on LC-QuAD 1.0 and WebQSP-WD.
%We also described a temporal KBQA system \system~that serves as a baseline on the dataset.  
%Future extenstions include improvement of the baseline approach for generalizable temporal QA.

==> TempQA-AAAI2022(2)/text/data.tex <==
    \section{TempQA-WD Dataset}
\label{sec:dataset}
 %\textit{TempQuestions} \cite{jia2018a}, a benchmark dataset for temporal KBQA is created by extracting temporal questions from three different KBQA datasets: 
In order to evaluate our approach on temporal reasoning, specifically on DBpedia and Wikidata as KGs, we require a dataset to be based on one of these two KGs. \textit{TempQuestions} \cite{jia2018a} is the first KBQA dataset intended to focus specifically on temporal reasoning. However, TempQuestions is based on Freebase.% it consists of temporal questions from three different KBQA datasets; \textit{Free917} \cite{cai2013}, \textit{WebQuestions} \cite{berant2013} and \textit{ComplexQuestions} \cite{bao2016}. %This was the first attempt at emphasizing and encouraging temporal reasoning for KBQA. 
 %In order to have a temporal QA dataset that can be:  (a) generalizable benchmark with parallel annotations on multiple knowledge bases; (b) up-to-date knowledge base such as Wikidata; and (c) intermediate evaluation with SPARQL queries, we decided to adapt \textit{TempQuestions} to Wikidata. 
 We adapt \textit{TempQuestions} to Wikidata\footnote{Creating a parallel dataset on two KGs (DBpedia and Wikidata) is non trivial and labor intensive. Therefore, we opted to create a dataset based on Wikidata alone since it is the most up-to-date KG.} to create a temporal QA dataset that has three desirable properties. First, we create a generalizable benchmark that has parallel answer annotations on two KBs. Second, we take advantage of Wikidata's evolving, up-to-date knowledge. Lastly, we enhance \textit{TempQuestions} with SPARQL queries which was missing in original dataset. We also add entity, relation, intermediate lambda expression annotations for a subset of the dataset that are used by the~\system.
 
 
 %However, the gold answers for these datasets are based on \texit{Freebase} which was officially discontinued from year $2014$ \cite{freebase}. 
 
 %It is desirable to have a benchmark dataset, especially for temporal questions, on a KB that is up to date, and not frozen in time. \textit{Wikidata} \cite{wikidata} offers a good option, as it is also better structured, apart from being more up-to-date and evolving.

%Instead of creating a new dataset with a fresh set of questions, we decided to adapt \textit{TempQuestions} dataset \cite{jia2018a} to \textit{WikiData}, as this also would easily serve the purpose of building a dataset with parallel annotations on multiple KBs (in our case two different KBs, i.e., \textit{WikiData} and \textit{Freebase}). As explained in the previous section, we believe this likely will play a role in helping drive research towards development of generalizable approaches, i.e., those that could be easily adaptable to multiple KBs. \pavan{We need to emphasize the TempQuestions does not have SPARQL queries where as having an intermediate representation would allow 1. Allow KG independent research }

%There has been attempts to transfer KBQA questions to \textit{WikiData} by WebQSP-WD~\cite{} and SimpleQuestions-WD~\cite{}. They directly map the answers of Freebase to their corresponding entity in Wikidata. However, this has multiple challenges: 
There has been two previous attempts at transferring Freebase-QA questions to \textit{Wikidata}; namely WebQSP-WD~\cite{webqsp} and SimpleQuestions-WD(SWQ-WD)~\cite{diefenbach2017wdaqua}. 
SWQ-WD contains only single triple questions whereas WebQSP-WD have only the final question answers that map directly to corresponding entities in Wikidata. However, as stated ~\cite{webqsp}, one challenge is that not all \textit{Freebase} answers can be directly mapped to entities in \textit{Wikidata}. For example, the Freebase answer annotation for the question ``When did Moscow burn?''  is ``1812 Fire of Moscow'', despite the year being entangled with the event itself. In contrast, Wikidata explicitly represents the year of this event, with an entity for ``Fire in Moscow'' and an associated year of ``1812''. Thus, a direct mapping between the two answers is not possible, as it would amount to a false equivalence between ``1812 Fire of Moscow'' and ``1812''.
%For example, the question "When did Moscow burn?" has freebase answers "1812 Fire of Moscow" that cannot be directly transferred/verified in Wikidata because the entity of relevance on Wikidata is "Fire in Moscow" with answer being "1812". adopting the directly mapping strategy suggested by \cite{} for temporal questions might lead to incomplete or incorrect answers hence affecting the evaluation of different systems. For instance, a question "when is the last time the Giants won the World Series?" has freebase answers as "2012 World Series". On the other hand, Wikidata has updated information for this question with answer being "2014". This is primarily because the dataset is old and the freebase as a knowledge base is outdated. 
%However, this has multiple challenges: 
%\begin{itemize}
%\item As stated in ~\citet{}, one challenge is that not all \textit{Freebase} answers can be directly transferable to \textit{Wikidata}. For example, the question "When did Moscow burn?" has freebase answers "1812 Fire of Moscow" that cannot be directly transferred/verified in Wikidata because the entity of relevance on Wikidata is "Fire in Moscow" with answer being "1812". \item adopting the directly mapping strategy suggested by \cite{} for temporal questions might lead to incomplete or incorrect answers hence affecting the evaluation of different systems. For instance, a question "when is the last time the Giants won the World Series?" has freebase answers as "2012 World Series". On the other hand, Wikidata has updated information for this question with answer being "2014". This is primarily because the dataset is old and the freebase as a knowledge base is outdated. 
%\end{itemize}

In order to address such issues, %we opted to take on the tedious task of manually writing SPARQL queries, 
we enlisted a team of annotators to manually create and verify SPARQL queries, %which allows for answers'  verification and updates as and when there are periodic updates on Wikidata. 
ensuring not only that the SPARQL formulation was correct, but that the answers accurately reflected the required answer type (as in the ``Fire in Moscow'' example above) and the evolving knowledge in Wikidata.
% (as the Freebase answers from the original dataset may be outdated). 
Having SPARQL queries also facilitates intermediate evaluation of the approaches that use semantic parsing to directly generate the query or the query graph, %~\cite{ijcai2020}, 
increasing interpretability and performance in some cases~\cite{webqsp}. 
%At the minimum, manually written SPARQL queries on \textit{WikiData} are needed for each question, in order to verify if the answer is present or not, and note down if available. 
%Writing SPARQL queries need manual search within the KB for matching entities/predicates and navigating around to estimate the reasoning required to be encoded in the SPARQL. Some questions could fall-out in this process depending upon non-availability of the answers or unavailability of the required reasoning paths. 
% However, given that we are considering temporal questions, presence of necessary time interval information about events on Wikidata is critical, which is not always the case.
%Next, we give a brief overview of how \textit{Wikidata} is organized, before explaining the dataset creation process.
% Before we get into dataset details, we give a brief overview of how \textit{Wikidata} is organized as some of its representational conventions impact our dataset creation process.

\input{text/data/wikidata}
\input{text/data/data_details}
%\input{text/data/lambda}

%\input{text/data/analysis}


==> TempQA-AAAI2022(2)/text/data/data_details.tex <==
\noindent
\textbf{Dataset Details}
\begin{table}[ht]
\begin{small}
\centering
\begin{tabular}{c|c|c|c}
\toprule
Dataset & Size & Answer & Add'l Details \\
% & & & \\
\midrule
\textit{TempQuestions(Freebase)} & 1271 & \textit{Freebase} & A \\
\midrule
\textit{TempQA-WD (Wikidata)} & 839 & \textit{Wikidata} & A + B \\
\midrule
\textit{A Subset of TempQA-WD} & 175 & \textit{Wikidata} & A + B + C \\
\bottomrule
\end{tabular}
\caption{Benchmark dataset details. \textit{TempQuestions} denote original dataset with \textit{Freebase} answers \cite{jia2018a}. Second row is the subset adapted to \textit{Wikidata} and the third row is the \textit{devset} taken out of it.
%The remaining two, i.e., \textit{testset} and \textit{devset}, are part of the benchmark dataset we created with \textit{WikiData} answers. In column titled \textit{Add'l Details}: 
Set-A denote \textit{TempQuestions} with- \{temporal signal, question type, data source\}. Set-B -\{Wikidata SPARQL , answer, category\}. Set-C-\{AMR, $\lambda$-expression, entities,  relations, KB-specific $\lambda$-expression\} }
\label{tab:benchmark}
\end{small}
\end{table}
Table~\ref{tab:benchmark} gives details of our new benchmark dataset. We took all the questions from \textit{TempQuestions} dataset (of size $1271$) and chose a subset for which we could find \textit{Wikidata} answers. This subset has 839 questions that constitute our new dataset, \dataset. We annotated this set with their corresponding \textit{Wikidata} SPARQL queries and \textit{Wikidata} answers. We also retained the \textit{Freebase} answers from the \textit{TempQuestions} dataset effectively creating  parallel answers from two KBs. Additionally, we  added a question complexity label to each question, according to the reasoning complexity required to answer the question. Details of categorization are present in supplementary material. Within this dataset, we chose a subset  of $175$ questions for detailed annotations as described in Set-C in the table description leaving $664$ question as test set. %Details of those additional annotations can be found in the Caption of Table~\ref{tab:benchmark} and an  %\colorbox{yellow}{an} 
%illustration of such annotations for a sample question can be found in Figure~\ref{fig:example}. 
 %{\color{red}can be found in the caption} of Table~\ref{tab:benchmark}. \pavan{Can you please add more information on what the detailed annotations are with example?}. 
%The goal of these additional annotations is to encourage building modular KBQA systems that have improved interpretability, i.e., to evaluate accuracy of outputs expected at intermediate stages of the system. 
%We believe these additional annotations are potentially useful to evaluate modular approaches for KBQA. 
%Modular approaches such as \cite{pavan2020} are more appropriate for KBQA, given difficulty in gathering large amount of training data to build end-to-end systems. In fact, our baseline system \system, described in Section \ref{sec:baseline}, to evaluate with benchmark dataset is also a modular approach. Such approaches stack together, in a pipeline, various modules built elsewhere with minimal adaptation.
%In such a setup, it is important to evaluate outputs at intermediate stages of the pipeline. Additional annotations include, ground truths for intermediate meaning representations such as AMR, $\lambda$-expression of the question and KB-specific $\lambda$-expressions, and mention-of/KB-specific entities and relations. 
%We also categorized questions into Simple, Medium, Complex based on the temporal and other reasoning requirements it has. More details about these categorization are presented in the supplementary material.

% \subsubsection{Question Complexity Categorization}
% \label{sec:category}
% \begin{table}[htb]
% \begin{small}
% \centering
% \begin{tabular}{l|l}
% \toprule
% % \hline
% \begin{tabular}[l]{@{}l@{}}
%     \textbf{Category}\\
%     \textbf{(dev/Test)}
% \end{tabular} 
% & 
% \textbf{Example} \\
% \midrule
% % \hline

% \begin{tabular}[l]{@{}l@{}}
%     Simple\\
%     (92/471)
% \end{tabular} 
% & 

% \begin{tabular}[c]{@{}l@{}}

% {\bf who is the governor of Hawaii now?}\\
% SELECT ?a WHERE \{ \\
%     wd:Q5589655 wdt:P1308 ?a \}\\
    
%     \end{tabular} \\
% \hline
% \begin{tabular}[l]{@{}l@{}}
%     Medium\\
%     (71/154)
% \end{tabular} 
% & 

% \begin{tabular}[c]{@{}l@{}}

% {\bf who was the US president} \\
% {\bf during cold war?   }\\
% SPARQL in Figure~\ref{fig:example} \\

%   \end{tabular} \\
% \hline
% \begin{tabular}[l]{@{}l@{}}
%     Complex\\
%     (12/39)
% \end{tabular} 
% & 
% \begin{tabular}[c]{@{}l@{}}

% {\bf who was president of the us when }\\
% {\bf douglas bravo was a teenager? } \\
% SELECT DISTINCT ?a WHERE \{\\
%   ?a p:P39 ?e. \tab
%   ?e ps:P39 wd:Q11696.\\
%   ?e pq:P580 ?st1.\tab
%   ?e pq:P582 ?et1.\\
%   wd:Q4095606 wdt:P569 ?x.\\
%   bind ((?x + "P13Y"$^\wedge^\wedge$xsd:duration) as ?st2)\\
%   bind ((?x + "P19Y"$^\wedge^\wedge$xsd:duration) as ?et2)\\
%   FILTER (?st1<=?et2 \&\& ?st2<=?et1) \}\\
% \end{tabular} \\

% \bottomrule
% \end{tabular}
% \caption{Examples of Simple, Medium, and Complex temporal reasoning question in the dataset.}
% \label{tab:complexity_examples}
% \end{small}
% \end{table}




% For evaluations in Section~\ref{sec:eval}, we divided dataset \dataset~of size $839$ into two parts,\dataset-test of size $664$ and \dataset-dev of size $175$. In fact, \dataset-dev is that part of the dataset with fine-grained annotations. 
% In this dataset, we also labeled questions with complexity category based on the complexity of the question in terms of temporal and non temporal reasoning required to answer. Table~\ref{tab:complexity_examples} shows the examples for each category of complexity defined below.
% \vspace{0.1cm}
% %\begin{itemize}
% %\item 

% \noindent \textbf{1) Simple:} Questions that involve one temporal event and need no temporal reasoning to derive the answer. For example, questions involving simple retrieval of a temporal fact or simple retrieval of other answer types using a temporal fact. 

% %\item 
% \noindent \textbf{2) Medium:} Questions that involve two temporal events and need temporal reasoning (such as overlap/before/after) using time intervals of those events. We also include those questions that involve single temporal event but need additional non-temporal reasoning.


% %\item 
% \noindent \textbf{3) Complex:} Questions that involve two or more temporal events, need one temporal reasoning and also need an additional temporal or non-temporal reasoning like teenager or spatial or class hierarchy.

% %Table~\ref{tab:complexity_examples} shows number of dev and test questions for each category along with an example question and its SPARQL query.
% %\end{itemize}




% %Data and annotation details:
% %* TempQA - 1272
% %      - Ques + GT Freebase Ans + temporal signal + question type + data source
% %* Our test - 500 
% %      -  Ques + GT Wikidata SPARQL + GT WikiData Ans + Complexity Categories + metadata from orig. data.
% %* Our dev - 175
% %      - similar info as above + GT AMR + GT Lambda Expression + GT WikiData entities/relations + GT KB-Specific Lambda

% %Complexity categorization of question with respect to Wikidata.
% %1) Simple - Single temporal event with no temporal reasoning required - simply retrieving a temporal fact / retrieving answer based on a single temporal fact.
% %2) Medium - Two temporal events and a temporal reasoning across events like overlap, before after case / single temporal event together with additional non-temporal reasoning.
% %3) Complex - Two or more temporal events  - with additional temporal events like teenager / including additional spatial reasoning or class hierarchy reasoning.

==> TempQA-AAAI2022(2)/text/data/lambda.tex <==
\textbf{Lambda Calculus}
%Although deriving KB-specific query of a NL question is the end goal of KBQA system, it is useful to also look the intermediate meaning representations of the questions. 
%For example, modular approaches, like our baseline described in Section \ref{sec:baseline}, would generate such intermediate representations. We use $\lambda$-expression for this purpose.
%For this, we use $\lambda$-calculus based logical representation of the question, i..e, $\lambda$-expression of the question.
%This is modular approaches are to likely need to attractive alternatives \cite{pavan2020}, given difficulty in building end-to-end systems that need large amount of training data.
%Modular approaches stack together, in a pipeline, various modules that are built elsewhere and typically need only minimal adaptation.
%In this context, for our dataset, it is useful to not only have the annotations for the end goal of KB-specific queries, but also have annotations for the intermediate outputs of different modules. These include modules that output intermediate meaning representations. 
%Here, we give a brief description of $\lambda$-calculus, since we use $\lambda$-expressions to logically represent the semantics of questions.
$\lambda$-calculus, by definition, is considered the smallest universal programming language that expresses any computable function.
%In our pipeline Lambda calculus plays vital role in representing intermediate logical form of question. By definition, $\lambda$ calculus is smallest universal programming language as it facilitates to express any computable function using its formalism. It mainly focuses on applying transformation rules to express computable function. 
In particular, we have adopted \textit{Typed} $\lambda$-\textit{Calculus} presented in \cite{zettlemoyer2012learning} which support addition of new higher order functions necessary for handling various reasoning types. %We demonstrate this for temporal reasoning. 
%In our representation we have used Constants, Logical Connectives similarly. However, we have introduced some new temporal quantifiers and instance variable in lambda expression to avoid function nesting.
We use constants and logical connectives like AND, OR, NEGATION and functions like argmin, argmax, count, etc., presented in this work. Apart from this, we also added new temporal functions to demonstrate the system's adaptability to support new reasoning types.
For example, consider the following question and its corresponding logical form:  
\begin{center}
\begin{tabular}{l c}
 Question: & When was Barack Obama born?\\ 
 Logical Form: & \begin{tabular}{l l}$\lambda$\textit{t. born(b,``Barack Obama")} $\wedge$\\\textit{interval(t, b)} \end{tabular}\\  
\end{tabular}
\end{center}
Here, \textit{b} is instance variable for event \textit{born(b, ``Barack Obama")} and \textit{interval(t, b)} finds time for the event denoted by \textit{b}. Variable \textit{t} is unknown which is marked as $\lambda$ variable.

%Consider the example question text and its logical form. In logical form, \textit{b} is instance variable for \textit{born(b,``Barac Obama")}. \textit{interval(t, b)} finds time for event \textit{b}. Variable \textit{t} is unknown which is marked as lambda variable.
%\subsubsection{Temporal Functions:}
\noindent
\textbf{Temporal Functions:} We introduce \textit{interval, overlap, before, after, teenager, year}; where \textit{interval} gets time interval associated with event and \textit{overlap, before, after} are used to compare temporal events. \textit{teenager} gets teenager age interval for a person, and \textit{year} return year of a date.\footnote{Although there are many other possible temporal functions for specific English words, such as \textit{adult} and \textit{tween}, we defined \textit{teenager} because it was featured in the datasets explored here.}
% We have adopted following $\lambda$ calculus grammar from \cite{Rojas15}:
% \begin{center}
% \begin{tabular}{l l l}
%  <expression>&:=&\begin{tabular}{l l}<name> | <function> |\\<application> \end{tabular}\\ 
%  <function>&:=&$\lambda$<name>.<expression>\\  
%  <application>&:=&<expression><expression>\\
% \end{tabular}
% \end{center}
% Notice that, \textit{expression} is main concept in $\lambda$ calculus, however our usage is limited to function only. We have skipped detailed description of grammar as it is widely known and available.

%$\lambda$t. born(b,``Barac Obama")$\wedge$time(t, b)


==> TempQA-AAAI2022(2)/text/data/wikidata.tex <==
% \subsection{Wikidata}
% Wikidata%\footnote{https://www.wikidata.org/} 
%     is a free knowledge base that is actively updated and maintained. It has 94.97 million data items as of September, 2021 and continuously growing each day with permission for volunteers to edit and add new data items. We chose Wikidata as our knowledge base as it has many temporal facts with appropriate knowledge representation encoded. %embedded with the statements in the form of reified statements, making it an interesting KB for testing temporal question answering. 
% It supports reification of statements (triples) to add additional metadata with qualifiers such as start date, end date, point in time, location etc. 
% %to capture valid time interval of the statement, location where the event has occurred or any other details that are relevant to the system. 
% %Figure~\ref{fig:temporal_reasoning_example} shows an example of reified temporal information assocaited to entities Joe Hart and Manchester City. 
% %With such representation and the availability of up-to-date information, Wikidata makes it a good choice to build benchmark datasets to test different kinds of reasoning including temporal reasoning.
% Figure~\ref{fig:example} shows the event node \texttt{?e1} associated with a person having the position of US President and how the start time (\texttt{?st1}) and end time (\texttt{?et1}) can be reached from that node.
% %\vspace{-0.2cm}
% % \begin{figure}[t]
% %   \centering
% %   \includegraphics[scale=0.36]{./figures/WikidataExample.pdf}
% %   \caption{An illustration of Wikidata Reification.}
% %   %\vspace{-0.2cm}
% %   \label{fig:temporal_reasoning_example} 
% % \end{figure}


==> TempQA-AAAI2022(2)/text/eval.tex <==
\section{Evaluation}
\label{sec:eval}
\begin{table*}[tb]
\centering
\small
\begin{tabular}{l|ccc|ccc|ccc|ccc|ccc}
\toprule
KB~~~~~~~~~~~~~$\rightarrow$ & \multicolumn{6}{|c|}{DBpedia} & \multicolumn{9}{|c}{Wikidata} \\ 
\midrule
DataSet~~~~~~$\rightarrow$& \multicolumn{3}{|c|}{LC-QuAD 1.0} &\multicolumn{3}{|c|}{QALD-9} &\multicolumn{3}{|c|}{WebQSP-WD} & \multicolumn{3}{|c|}{SWQ-WD} &\multicolumn{3}{|c}{ TempQA-WD}\\
 Reasoning~~$\rightarrow$& \multicolumn{3}{|c|}{multi-hop} &\multicolumn{3}{|c|}{multi-hop} &\multicolumn{3}{|c|}{multi-hop} & \multicolumn{3}{|c|}{single-hop} &\multicolumn{3}{|c}{ Temporal}\\
\hline
System~~$\downarrow$ & P & R & F1 & P & R & F1& P & R & F1& P & R & F1& P & R & F1 \\
\hline
WDAqua   &  0.22 & 0.38  &  0.28  & 0.26 & 0.26 & 0.25 & - & - & - & - & - & - & - & - & - \\
gAnswer   & -  & - & - &  0.29 &   0.32   & 0.29 & - & - & - & - & - &- & - & - & - \\
QAMP   & 0.25 & 0.50 &  0.33  & - & - & - & - & - & - & - & - &- & - & - & - \\
NSQA   & 0.44 &  0.45   & 0.44  & \bf 0.31 & \bf 0.32 & \bf 0.31&  - & - & -  & - & - &- & - & -  & - \\
GGNN   & - &  -   & -  & - & - & - &   0.27 & 0.32 & 0.26  & - & - &- & - & -  & - \\
\system  & \textbf{0.47} &\textbf{0.48}  & \textbf{0.47} & 0.29 & 0.30 & 0.29  & \textbf{0.32}& \textbf{0.36}& \textbf{0.31} &0.42 &0.55 &0.44 & 0.32 & 0.34 & 0.32  \\
\bottomrule
\end{tabular}
\caption{ \system's Performance across knowledge bases and reasoning types. Baseline numbers are taken from \citet{pavan2020} and \citet{C18-1280}. P-Precision, R-Recall}
\label{table:results}
\end{table*}
\input{text/eval/setup}
\input{text/eval/datasets}
\input{text/eval/metrics}
\input{text/eval/results}

==> TempQA-AAAI2022(2)/text/eval/datasets.tex <==

\subsubsection{Datasets:}
\label{sec:data}
%\begin{table}[htb]
%\begin{center}
%\small
%\begin{tabular}{|l|ll|}
%\hline
%  Dataset  & Dev & Test  \\
%\hline
% TempQA-WD   &    175       & 664       \\
%SWQ-WD &  200       & 5622       \\
% WebQSP-WD &       200     & 1033   \\
%\hline
%\end{tabular}
%\caption{Datasets }
%\label{table:datasets}
%\end{center}
%\end{table}
We considered two different KBs namely DBpedia and Wikidata to evaluate our system. We did not consider Freebase as its no longer actively maintained and is not up-to-date. 
Along with the new benchmark dataset \dataset~introduced in this paper, we also evaluate our baseline system on two other benchmark datasets adopted to Wikidata, to evaluate its effectiveness beyond temporal questions. They are SWQ-WD%\footnote{https://github.com/askplatypus/wikidata-simplequestions}
~\cite{wikidata-benchmark}, which consists of 14894 train and 5622 test set questions, and WebQSP-WD
%\footnote{https://github.com/UKPLab/coling2018-graph-neural-networks-question-answering}
~\cite{C18-1280}, which consists of 2880 train and 1033 test set questions.
%Dev/test sizes of SWQ-WD 200/5622, WebQSP-WD 200/1033. 
For DBpedia, we used QALD-9~\cite{QALD_2017}, that has 408 training and 150 test questions, and LC-QuAD 1.0~\cite{trivedi2017lc} data set, that has 4k training set and 1k test set. Each of these datasets operate on their own version of the DBpedia and SPARQLs provided and we used the same instance of DBpedia for evaluation.
%Table~\ref{table:datasets} gives the details of dev and test splits used. 
The baseline system is tuned with dev sets of 175 from TempQA-WD and 200 from SWQ-WD train and 200 from LC-QuAD 1.0 and evaluated on all the the five test sets. %We also have 100 dev from QALD and 200 dev from WebQSP-WD. %As pointed by the authors of WebQSP-WD, the dataset is not validated to verify if the question is answerable on Wikidata and if the gold answers are up-to-date with respect Wikidata answers. Our analysis on a subset of $200$ dev questions found that $85$ of the questions had ground truth issue with respect to Wikidata.
%with either answer being different as per Wikidata or more answers being present than what came from Freebase or supporting facts not being present in the Wikidata to answer them. Performance on this dataset need to be interpreted keeping this issue in mind.



==> TempQA-AAAI2022(2)/text/eval/metrics.tex <==
%\subsubsection{Metrics}
%We use the standard macro precision, macro recall and F1 measures normally used to benchmark the KBQA systems. All the numbers produced are using GERBIL by providing the gold answers and system generated answers to it.
%We use GERBIL%\footnote{https://github.com/dice-group/gerbil}
%~\cite{DBLP:journals/semweb/UsbeckRHCHNDU19} to compute performance metrics from the pairs of gold answers and system generated answers from the pipeline.
%We use standard performance metrics typically used for KBQA systems, namely macro precision, macro recall and F1.


\subsubsection{Baselines}
We Compare ~\system~ with various KBQA baseline systems as given in Table~\ref{table:results}. To our knowledge there is no other system that works across both DBpedia and Wikidata. We took the numbers reported from NSQA~\cite{pavan2020} work, which is current state-of-the-art on both LC-QuAD 1.0 and QALD-9 datasets. We also compare our work with GGNN~\cite{webqsp} which is the only known benchmark for WebQSP-WD dataset. We also compare our work with WDAqua~\cite{diefenbach2017wdaqua}, gAnswer~\cite{gAnswer} and QAMP~\cite{qamp} systems. %For other SWQ-WD dataset, to our knowledge there is no known benchmark. We provide our baseline numbers from the system for both SWQ-WD and TempQA-WD dataset introduced in this paper.

==> TempQA-AAAI2022(2)/text/eval/results.tex <==
\subsection{Results \& Discussion}

Table~\ref{table:results} shows performance of \system ~on two different KBs with five different datasets described in Section \ref{sec:data}. We also show the type of reasoning required for each dataset along with the precision/recall and F1 measure.
We use GERBIL%\footnote{https://github.com/dice-group/gerbil}
~\cite{DBLP:journals/semweb/UsbeckRHCHNDU19} to compute performance metrics from the pairs of gold answers and system generated answers from the pipeline.
%We selected these datasets as they have more natural questions.
%{\achille{We should also report results from other QA systems operating on Wikidata on the three datasets or say explicitly that no such comparable systems exist }}
%This table also shows performance of  TEQUILLA%\footnote{https://tequila.mpi-inf.mpg.de/}
%~\cite{jia2018b} (that uses Freebase as its underlying KB) on \dataset ~test set.
To our knowledge, ours is the first system reporting KBQA numbers across two different KBs and varying reasoning types. We get state of the art numbers beating NSQA~\cite{pavan2020} on LC-QuAD 1.0 and also achieve comparable numbers for QALD. For WebQSP-WD dataset we get state of the art numbers nearly $20\%$ gain over GGNN~\cite{webqsp}.
%Please note that we haven't support for handling comparative, superlative questions in our system which are prominent in QALD.
%temporal QA performance on Wikidata.
The accuracy numbers for Wikidata datasets show that there is ample scope for improvement for different modules. This gets evident when we look at the module performances on a small set of development sets across datasets. For WebQSP-WD we did not have any ground truth for evaluating entity linking and relation linking. 
%We found several issue with the way this dataset 
%Table \ref{table:category} gives detailed report of performance for different categories of question complexity from our system on our newly introduced ~\dataset. 
%Next, we describe module performances on small development sets across different datasets followed by ablation study for TempQA-WD on Wikidata and LC-QuAD 1.0 on DBPedia.

%Performance of TEQUILLA reflects how well Accu and Quint (the QA systems it used) are adapted to Freebase.
%This in addition to the fact that majority of the questions fall under simple questions category (471 simple vs 39 complex as shown in Table~\ref{tab:complexity_examples}), it is able to achieve better accuracy on Freebase. Given relatively less focus of research on temporal QA on Wikidata so far, we believe our benchmark dataset would help accelerate more research and datasets in the future.
%\subsubsection{Individual Module Performance:} Here we describe the results of individual modules on small development set across different datasets is given below.

\noindent\textbf{\textit{AMR:}}
Table \ref{tab:amr_per} show the performance of the AMR parser on the 5 development sets in Smatch (standard measure used to measure AMRs) and Exact Match ($\%$ of questions that match fully with ground truth AMR).

\begin{table}[h]
\begin{small}
\centering
\begin{tabular}{l|c|c|c} 
\toprule
Dataset & KB & Smatch & Exact Match \\\midrule
LC-QuAD 1.0 & DBpedia & 87.6 & 30.0 \\
QALD-9 &   DBpedia & 89.3 & 41.8 \\
WebQSP-WD & Wikidata & 88.0 & 43.8 \\
SWQ-WD & Wikidata & 83.0 & 37.8 \\
TempQA-WD & Wikidata & 89.6 & 39.8 \\
\bottomrule
\end{tabular}
\caption{AMR parser performances on the development sets}
\label{tab:amr_per}
\end{small}
\end{table}

\noindent\textbf{\textit{Entity Linking:}}
Table \ref{EL_performance} below captures the performance of entity linking module on different datasets. The question level accuracy is computed by considering all the entities present in each question. However, mention level accuracy is computed by considering single mention at a time. We can see that entity linking performance for Wikidata datasets is low compared to DBpedia. One of the reasons for is all these datasets are adopted from Freebase dataset and the way entities represented in these two KBs is different. Also, very little research is done on entity linking for Wikidata and KBQA in general. 
\begin{table}[htb]
\begin{small}
\centering
\setlength\tabcolsep{6pt}
\renewcommand{\arraystretch}{1.0}
\begin{tabular}{lcrr}
\toprule
\multirow{2}*{Dataset}& \multirow{2}*{KB} & \multicolumn{2}{c}{Accuracy (\%)}  \\
& & Mention Level & Question Level \\
\midrule
LC-QuAD 1.0 & DBpedia & $86.81\;(91.94)$ &  $84.00\;(90.50)$\\
QALD-9 & DBpedia & $89.52\;(94.28)$ &  $89.79\;(93.87)$\\
TempQA-WD& Wikidata & $74.01\;(82.47)$  & $57.14\;(69.71)$ \\
SWQ & Wikidata & $72.27\;(83.18)$ &  $70.14\;(81.59)$\\
\bottomrule
\end{tabular}
\caption{Entity linking performance on development sets when gold mentions are provided. The numbers inside parentheses denote the Hits@5 scores.}
\label{EL_performance}
\end{small}
\end{table}

\noindent\textbf{\textit{Relation Linking:}} Table \ref{RL_performance} captures the performance of the relation linking module. It demonstrates that relation linking is still a challenging tasks specially with multi-hop reasoning and temporal reasoning, where the query graph is disconnected across events, there is room for improvement.    
%We ran TempQA-WD test set on TEQUILLA\footnote{https://tequila.mpi-inf.mpg.de/}~\cite{jia2018b} that uses Freebase as its underlying KB. %We Tuned our system using 175 dev questions from TempQA-WD and SWQ-WD datasets and ran the same pipeline to test on WebQSP-WD dataset as well. 
%We achieve better performance as~\cite{webqsp} (0.25) on the same test set without any tuning.
%of baseline and TEQUILLA systems on the on further categorization present in the dataset. Note that dataset is categorized purely based on the reasoning requirements and not based on individual component complexity like entity extraction linking or relationship linking etc. So, the numbers presented may not truly reflect the reasoning complexity depending on how the individual modules perform.

\begin{table}[htb]
\begin{small}
\centering
\setlength\tabcolsep{6pt}
\renewcommand{\arraystretch}{1.0}
\begin{tabular}{lcccc}
\toprule
Dataset & KB  & Precision & Recall & F1 \\
\midrule
LC-QuAD 1.0 & DBpedia & 0.52 & 0.50 & 0.50 \\
QALD-9 & DBpedia & 0.55 & 0.53 & 0.53 \\
TempQA-WD& Wikidata & 0.43 & 0.43 & 0.42 \\
SWQ & Wikidata & 0.67 & 0.68 & 0.67 \\
\bottomrule
\end{tabular}
\caption{Relation linking performance on development sets.}
\label{RL_performance}
\end{small}
\end{table}




\subsubsection{Ablation Study:}
To gain more insights on the performance, we also did an ablation study of \system~using \dataset~dev set for Wikidata and 100 question dev set from LC-QuAD 1.0 that we manually annotated with ground truth for all the modules. This shows the impact of individual module on overall performance is evaluated. Table~\ref{table:ablation} shows the results.
%We took intermediate ground truths available in that dataset and fed them directly as input %to appropriate modules in the pipeline, 
%to assess the impact of performance of different modules.
%We did similar study also with SWQ-WD dataset, however it has ground truth annotations only for AMR and entities. 
%In the table, row \textit{Machine} refer to full end-to-end performance without use of any ground truths. Rows GT-$Module$ are for the use of intermediate ground truths. 
For example GT-$AMR$ refers to the case where ground truth AMR is fed directly into $\lambda$-module. The table shows large jump in accuracy (in both the datasets) when fed with ground truth entities (GT-EL) and ground truth relations (GT-RL). This points to the need for improved entity linking and relation linking on both datasets across KBs.

%In Table~\ref{table:f1} also shows performance of \system~on SWQ-WD and WebQSP-WD datasets. For SWQ-WD there is no known baseline to our knowledge. For WebQSP-WD, accuracy of \system~is relatively better than GGNN~\cite{C18-1280} which achieves F1 of $0.26$. %A point to note here, as explained in Section~\ref{sec:data}, WebQAP-WD has only mapped Freebase answers to Wikidata which potentially might have introduced many errors in ground truths answers.

%Overall performance of the \system shows that there is scope
%From the table it can be seen that Entity linking and relation linking on Wikidata has scope for improvement. Wikidata also poses its own challenge in terms of reified statements that are not present in other datasets.

%Table~\ref{table:category} shows a break-up of the performance on TempQA-WD for different categories of question complexity as described in Section~\ref{sec:category}.

%by supplying the ground truth annotated for different modules in the 175 question dev set for TempQA-WD dataset. We also annotated ground truth AMR and entities for SWQ-WD dataset as well and the results using ground truth are reported. Here $Machine$ refers to running the pipeline end to end with machine generated output from each module. GT-$module$ refers to using ground truth until that module in the pipeline. GT-RL means running the pipeline with the ground truth for AMR, $\lambda$ expression, entity linking, relationship linking modules and machine generated output for other modules. Note that We only had ground truth AMR and Entities annotated for SWQ-WD dataset. From the ablation study it can be seen that Entity linking and relation linking on Wikidata  has lot of scope for improvement. Wikidata also poses its own challenge in terms of reified statements that are not present in other datasets.

% \begin{table}[htb]
% \small
% \begin{tabular}{l|llll}
% \toprule
%     System&  Dataset  & Precision & Recall & F1 \\
% \midrule
%  &TempQA-WD   &    0.34       &  0.32      &  0.32       \\
% \system &SWQ-WD &    0.54       &   0.43     &  0.44       \\
%  &WebQSP-WD &       0.32     &   0.29     &    0.28      \\
% \midrule
%  TEQUILLA&TempQA-FB  &    0.54      &    0.48   &   0.48      \\
% \bottomrule
% \end{tabular}
% \caption{Performance of our pipeline }
% \label{table:f1}
% \end{table}

% \begin{table}[htb]
% \small
% \begin{center}
% \begin{tabular}{l|llll}
% \toprule
%  System&Category & Precision & Recall & F1 \\
%  \midrule
%  &Simple  & 0.39 & 0.37 & 0.38               \\
%  \system &Medium  & 0.16 & 0.13 & 0.13                \\
%  &Complex  & 0.38 & 0.38 & 0.38               \\
% % \midrule
% %         & Simple  &    0.59     &    0.53  &   0.53      \\
% % TEQUILA& Medium &0.46 & 0.39& 0.40\\
% %     & Complex & 0.20&0.20 & 0.18\\
% \bottomrule
    
 
%  \end{tabular}
% \caption{Category wise Performance}
% \label{table:category}
% \end{center}
% \end{table}




%\begin{table*}[htb]
%\small
%\begin{tabular}{|llllllllll|}
%\hline
%    System&  Dataset  &Metric& %Machine & GT-AMR & GT-$\lambda$ %& GT-EL &GT-RL& GT-KB$\lambda$& %GT-SPARQL \\
% \hline
% & &Precision  &0.49 & 0.51&0.53 %& 0.61&0.92 & 0.93& 1.0    \\
%OurSystem&TempQA-WD &Recall  & 50.47&0.49 &0.52 & 0.60& 50.92&0.92 & 1.0    \\
%& &F1  & 0.47& 0.50&0.52 & 0.60& %0.92& 0.92&1.0     \\
% \midrule
% & &Precision  & 0.47&0.58 & - & %0.82& - & - & 1.0    \\
%OurSystem &SWQ-WD &Recall  &0.47 %&0.59 & - &0.82 & - & - & 1.0    %\\
%& &F1  &0.47 & 0.58& - & 0.82& - %& - &1.0     \\
%\hline
%\end{tabular}
%\caption{Ablation Study on the %Dev Set }
%\label{table:ablation}
%\end{table*}

\begin{table}[htb]
\small
\begin{tabular}{l|ccc|ccc}
%\begin{tabular}{|llllllllll|}
\toprule
& \multicolumn{3}{|c|}{TempQA-WD} & \multicolumn{3}{|c}{LC-QuAD 1.0} \\
\midrule
 & P & R & F1 & P & R & F1 \\
\midrule
NO GT & 0.47 & 0.50 & 0.47 & 0.50 & 0.52 & 0.50 \\
GT-AMR & 0.50 & 0.51 & 0.50 & 0.51 & 0.53 & 0.51 \\
GT-$\lambda$ & 0.52 & 0.53 & 0.52 & 0.52 & 0.53 & 0.52   \\
GT-EL & 0.60 & 0.62 & 0.60 & 0.63 & 0.66 & 0.64 \\
GT-RL & 0.92 & 0.93 & 0.92 & 0.99 & 0.98 & 0.98 \\
GT-KB-$\lambda$ & 0.93 & 0.93 & 0.93 & 1.0 & 0.99 & 0.99 \\
GT-SPARQL & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 \\
\bottomrule
\end{tabular}
\caption{Ablation Study on \dataset~and LC-QuAD 1.0 dev sets. P-Precision, R-Recall}
\label{table:ablation}
\end{table}




==> TempQA-AAAI2022(2)/text/eval/setup.tex <==
\subsubsection{Implementation Details:}
We implemented our pipeline using a Flow Compiler%\footnote{https://github.com/IBM/flow-compiler}
~\cite{chakravarti-etal-2019-cfo} stitching individual modules exposed as gRPC services. We defined the ANTLR grammar to define $\lambda$-expressions.
%, that includes rules to capture basic predicates, logical connectives (like $and, or, not$), basic temporal operators (like $argmin, argmax, min, max$), temporal operators (like {\it interval, overlap, before, after, teenager, now, age}) and so on. 
KB-Specific $\lambda$-expression to SPARQL module is implemented in Java using Apache Jena%\footnote{https://jena.apache.org/} 
~SPARQL modules, to create SPARQL objects and generate the final SPARQL query that is run on target KB end point. %\footnote{https://query.wikidata.org/}. 
The rest of the modules are implemented in Python and are exposed as gRPC services.  
%We use GERBIL%\footnote{https://github.com/dice-group/gerbil}
%~\cite{DBLP:journals/semweb/UsbeckRHCHNDU19} to compute performance metrics using the gold answers and the system generated answers from pipeline.

==> TempQA-AAAI2022(2)/text/introduction.tex <==
\section{Introduction}
\label{sec:intro}
%Given a natural language question, the goal of Knowledge Base Question Answering (KBQA) systems is to reason and retrieve the answer based on the facts available in Knowledge Bases (KB). 
The goal of Knowledge Base Question Answering (KBQA) systems is to answer natural language questions by retrieving and reasoning over facts in Knowledge Base (KB).
While reasoning in KBQA is evolving as an important research direction, most existing datasets and research in this area have primarily focused on one-triple questions~\cite{bordes2015large} or multi-hop reasoning questions~\cite{lcquad2,berant2013} as illustrated in Table~\ref{tab:multi-hop}. 
Currently, there is a lack of approaches and datasets that address other types of complex reasoning, such as temporal and spatial reasoning.
In this paper, we focus on a specific category of questions called \textbf{temporal questions}, where answering a question requires reasoning about points and intervals in time. 
For example, to answer the question \textit{What team did Joe Hart play for before Man City?}, the system must retrieve or infer \textit{when} Joe Hart played for Man City, \textit{when} Joe Hart played for other teams, and which of the latter intervals occurred \textit{before} the former.

%\vspace{-0.2cm}
\begin{table}[htb]
\begin{small}
\centering
\begin{tabular}{|l|l|}
%\toprule
\hline
\begin{tabular}[l]{@{}l@{}}
    \textbf{Category}\\
\end{tabular} 
& 
\textbf{Example} \\
%\midrule
\hline

\begin{tabular}[l]{@{}l@{}}
    Single-Hop
\end{tabular} 
& 

\begin{tabular}[c]{@{}l@{}}

\emph{ Who directed Titanic Movie?}\\
{\bf SPARQL:}
select distinct ?a where \{\\
  wd:Q44578 wdt:P57 ?a\}\\

    \end{tabular} \\
\hline
\begin{tabular}[l]{@{}l@{}}
    Multi-hop\\
\end{tabular} 
& 

\begin{tabular}[c]{@{}l@{}}

\emph{ Which movie is directed by James Cameron }\\
\emph{ starring Leonardo DiCaprio?  }\\
{\bf SPARQL:}
select distinct ?a where \{\\
  ?a wdt:P57 wd:Q42574. \\
  ?a wdt:P161 wd:Q38111. \} \\
   \end{tabular} \\
\hline
\begin{tabular}[l]{@{}l@{}}
    Temporal
\end{tabular} 
& 
\begin{tabular}[c]{@{}l@{}}
\emph{ what team did joe hart play }\\
\emph{ for before man city?  }\\
{\bf SPARQL:}
in Figure~\ref{fig:example} \\
\end{tabular} \\
%\bottomrule
\hline
\end{tabular}
\caption{Examples of Single-hop, Multi-hop and Temporal reasoning questions on Wikidata.}
%\vspace{-0.2cm}
\label{tab:multi-hop}
\end{small}
\end{table}


%Therefore, clearly demonstrating the need for extending approaches for other types of reasoning such as temporal and spatial. 
%In order to extend the scope of reasoning in KBQA, 
%This needs understanding of the question in terms of the knowledge as available in the KB. In specific, they map question to a KB-specific query, that when executed over the KB would derive the answer \cite{berant2013, svitlana2019, pavan2020}. 
%For this they: 1) map terms in the question to KB elements (i.e., entities and predicates) and 2) perform reasoning to infer answer from the facts as in the KB. Different questions have different reasoning requirements, depending upon the question complexity and the available KB facts. For example, possible KB-specific queries for question \textit{Country of Obama's birth?} include \textit{birthCountry("Obama", ?X)} or \textit{birthCity("Obama", ?Y) \& locatedIn(?Y, ?X)}. The $2^{nd}$ query performs multi-hop reasoning. 
%In this paper, we present a KBQA dataset focused on \textbf{temporal questions}, where reasoning to derive answers involve at least one step of temporal reasoning \cite{jia2018a, jia2018b} i.e., a manipulation of time intervals of the associated events. For example, as shown in Table~\ref{tab:temporal_reasoning_example}, the question \textit{What team did Joe Hart play for before Man City?}, requires knowing the time intervals of teams which Joe Hart played for and picking the one just before Man City.
%\textit{Who became president of France after ww2?}.


 
%Temporal Question Answering over knowledge bases is heavily impacted by the lack of datasets for evaluating the systems. 
%\vspace{-0.2cm}
Progress on Temporal KBQA is hindered by a lack of  datasets that can truely assess temporal reasoning capability of existing KBQA systems.
To the best of our knowledge, \textit{TempQuestions}~\cite{jia2018a} is the only available dataset for evaluating purely this aspect. It  has, however, a number of drawbacks: (a) the dataset uses Freebase~\cite{freebase} as the knowledge base, which is no longer maintained and  was officially discontinued in $2014$~\cite{freebase}; (b) the dataset contains only question-answer pairs and not their intermediate SPARQL queries which could be useful in  evaluating interpretability aspect of KBQA approaches based on semantic parsing ~\cite{yih2014semantic}; (c) unlike regular KBQA datasets~\cite{lcquad2, swq, azmy-etal-2018-farewell} that can attest KBQA generality over multiple knowledge bases such as DBpedia, and Wikidata, \textit{TempQuestions} is suited for a single KB.% In particular, to the best of our knowledge, there is no benchmark dataset for temporal questions with parallel annotations on multiple KBs.

%Past work on KBQA vary in terms of the core approach being used, that range from dependency parse-based approaches \cite{zou2014, sun2020b} to those involving end-to-end learning \cite{sun2020a, verga2020}. Many of these approaches use single KB as their knowledge source. Moreover, many of the datasets used for evaluation of these approaches are also single KB specific, such as Freebase or DBpedia. These factors are likely to have limited the generalizability of those approaches to other KBs \cite{dennis2018}. New datasets have recently been released with parallel annotations on multiple KBs \cite{lcquad2, swq, webqsp}, thus offering opportunity for generalizability across KBs. However, such datasets for complex questions are rare. 
 Our aim in this paper is to fill the above mentioned gaps by adapting the \textit{TempQuestions} dataset to Wikidata and by enhancing it with additional SPARQL query annotations. %Specifically, since \textit{TempQuestions} dataset contains complex temporal reasoning questions but on Freebase, we reused the natural language questions to create a temporal qa dataset  for WikiData~\cite{} as the Knowledge Base.
 %This would easily serve the purpose of building a dataset with parallel annotations on multiple KBs (in our case two different KBs, i.e.,WikiData and Freebase). 
 Having SPARQL queries for temporal dataset is crucial to refresh ground truth answers as the KB evolves.
We choose Wikidata for this dataset because it is well structured, fast evolving, and the most up-to-date KB, making it a suitable candidate for temporal KBQA.
Our resulting dataset thus contains parallel annotations (on both Wikidata and Freebase). This will help drive research towards development of generalizable approaches, i.e., those that could be easily be adaptable to multiple KBs.
In order to encourage development of interpretable, semantic parsing-based approaches, we (1) annotate the questions with SPARQL queries and answers over Wikidata, and (2) annotate a subset of this dataset with intermediate representations for the entities, relations, $lambda$-expression along with SPARQL needed to answer the question.
%with information necessary for evaluating entity linking, relation linking, and intermediate sparql representation that are necessary components of a KBQA system.  

 
 %a subset of this dataset is also annotated with outputs expected at various intermediate stages of the pipeline.

%In this paper, we also describe a neuro-symbolic approach to temporal KBQA. Although, primary goal of this approach is to simply serve baseline for the dataset described above, it has design level novelty guided by the requirements of interpretability and generalizability\pavan{I dont think we evaluate this aspect so calling it out as novelty might not be the best idea}. It includes a novel question understanding framework, where an intermediate KB-agnostic logic representation of the question is obtained first, followed by mapping onto a KB-specific logic representation that further could be executed over KB as SPARQL queries.

The main contributions of this work are as follows:
%\vspace{-0.2cm}

\begin{itemize}
     
     \item A benchmark dataset, called \dataset, for building temporal-aware KBQA systems on \textit{Wikidata} with parallel annotations on \textit{Freebase}, thus encouraging the development of approaches for temporal KBQA that generalize across KBs.
    \item SPARQL queries for all questions in our benchmark, with a subset of the data also annotated with expected outputs from intermediate stages of the question answering process, i.e. entity and relation linking gold outputs. The goal here is to encourage interpretable approaches that can generate intermediate outputs matching those fine-grained annotations. 
   \item A modular baseline approach, called \system, for temporal QA with novel question understanding framework to serve as a baseline for the benchmark dataset.
 \end{itemize}

%We first give details of the benchmark dataset in the next section, and then we describe baseline neuro-symbolic approach in the following section, followed further by discussions on experimentation and results.

%This involves understanding the NL question in terms of knowledge as available in the KB, in order to map that to a KB-specific query that when executed over the KB would derive the answer \cite{}. Depending upon the question complexity, this involves: 1) mapping of terms in the question onto KB elements (i.e., entities and predicates) and 2) reasoning to infer answer from the facts as found in the KB. For example, depending upon facts available in the KB, KB-specific queries for question \textit{Did Zinedine win 1998 football worldcup?} could be \textit{PersonWon("Zinedine Zidane", "1998 FIFA Worldcup")} or \textit{TeamMember("Zinedine Zidane", a) \& TeamWon(a, "1998 FIFA Worldcup")}. Reasoning in case of second query is multi-hop reasoning. % where facts considered to answer the question are inferred through composition of pairs of facts in the KB that are linked through common entity.
%Depending upon the type of the fact inferred, the reasoning step could be categorized as temporal, spatial and so on. For example, answering question \textit{Who became president of France after ww2?} would need temporal reasoning involving manipulation using time intervals. % since answer derivation would require looking into the time intervals of all the French presidents and choosing the one whose time interval is immediately after the time interval of 'World War 2'. 
%In this paper, our focus in on such kind of questions, called temporal questions, where at least one step of temporal reasoning is needed to derive the answer \cite{}.
%focus of this paper is on temporal question. 

%Past work on KBQA vary in terms complexity of the questions being addressed, with recent approaches addressing more complex questions. Recent work on temporal-specific KBQA include \cite{}. Past work also vary in terms of the core approach being adopted, ranging from dependency parse-based approaches to those involving end-to-end learning \cite{}. However, many of these approaches have focused on using single KB as their knowledge source \cite{}. Moreover, many of the datasets used for evaluation of these approaches are also single KB specific, such as Freebase or DBPedia \cite{}. These factors are likely to have resulted in limitations in the approach in terms of generalizability to other KBs. However, recently there are datasets made available with parallel annotations on multiple KBs, thus offering opportunities to explore KBQA approaches that are generalizable across KBs. But these cover only less complex questions. In particular, to our knowledge, there is no benchmark dataset for temporal questions with parallel annotations on multiple KBs. Our aim in this paper is to address this gap. In addition, in order to encourage the development of interpretable approaches, a subset of this dataset is also annotated with outputs expected at various intermediate stages of the pipeline.

%In this paper, we also describe a neuro-symbolic approach to temporal KBQA. The goal is to have this approach serve as a baseline approach for the dataset described above. With interpretability and generalizability being the guiding factors, this approach includes a question understanding framework where an intermediate KB-agnostic logic representation of the question is obtained first, followed by mapping onto a KB-specific logic representation that further could be executed over KB after mapping onto corresponding SPARQL queries.

%In the next section, we describe the benchmark dataset that we introduce. Then we describe the describe the neuro-symbolic approach that serve as a baseline for the dataset introduced. Followed by discussion on experimentation and results.

%One striking common feature of most of these approaches is that they are all built with goal of using a single KB (such as Freebase or DbPedia) as their knowledge source. As a result, it is hard to adapt models built using of these approaches to work on KBs other than what they are built for. In addition, datasets used to evaluate these approaches are also typically built using a single KB as knowledge source. On the other hand, datasets that  encourage development of approaches that are generalizable to multiple KBs with minimal effort  are highly desirable. In this paper, we present a benchmark dataset built towards this goal. In specific, we took a dataset that is built for Freebase and adapted a subset of that to build a parallel dataset for Wikidata. Existence of such dataset with parallel annotations would facilitate development of generalizable KGQA approaches that work on more than one KB. In addition, to encourage development of interpretable approaches we have annotated the dataset with outputs expected at intermediate various stages of the pipeline. In this paper we have chosen to focus on temporal question, and our plan is to extend this effort in the future to beyond temporal questions.




==> TempQA-AAAI2022(2)/text/introduction_pavan.tex <==
\section{Introduction}
\label{sec:intro}
%% KBQA is important but research has to be performed on a generalizable approach that is easily adaptable to different KBs and reasoning types.
The goal of Knowledge Base Question Answering (KBQA) systems is to answer natural language questions by retrieving and reasoning over facts in a Knowledge Base (KB). KBQA has gained significant popularity both due to its practical real-world applications and challenging research problems associated with it~\cite{fu2020survey}. However, most existing datasets and research in this area are primarily focused on \textit{single/multi-hop} reasoning on a \textit{single} knowledge base~\cite{trivedi2017lc,QALD_2017,yih-etal-2016-value}. 
Consequently, this has encouraged research in methodologies that are tuned to a restricted set of reasoning types on a single knowledge base, in turn lacking generalizability~\cite{pavan2020,zou2014natural,webqsp}. In this work, we propose a modular approach that is generalizable across knowledge bases and reasoning types.   

\begin{figure}[th]
  \centering
  \includegraphics[height=4.7cm,width=0.75\linewidth]{./figures/dbpedia_wikidata_ex.pdf}
  %\vspace{-0.35cm}
  \caption{A description of how information about Nero's predecessor is represented in DBpedia vs. Wikidata}
  \label{fig:query_graphs_comparison} 
\end{figure}

%% Why is generalization important and non trivial to a different KB. Talk about the representation that requires specific tuning for a new knowledge graph.
 Open Knowledge Bases such as DBpedia~\cite{auer2007dbpedia}, Wikidata~\cite{vrandevcic2014wikidata}, and Freebase~\cite{bollacker2008freebase} form the basis of many KBQA datasets. Each of these knowledge Bases, however, have different representations. For instance: information associated to the question \textit{``Who was roman emperor before Nero?"} from DBpedia and Wikidata are shown in Figure~\ref{fig:query_graphs_comparison}. We can see that Wikidata represents properties of facts such as replaces, temporal and spatial with reification.\footnote{Information about facts are explicitly mapped by making facts as primitive nodes.} On the other hand, DBpedia manages to represent it as a simple fact with the relationship to existing entity nodes. Handling such different representations is an unexplored challenge and requires to be addressed for a generalizable KBQA approach.%% Why is handling different reasoning types important and need generalizable thinking? 
  The second aspect where KBQA approaches fail to generalize is in handling complex reasoning types such as temporal and spatial reasoning. Table~\ref{tab:multi-hop} shows examples of questions that require different types of reasoning to answer them. Most research have focused on multi-hop reasoning questions~\cite{bordes2015large,lcquad2,berant2013}, lacking both approaches and datasets that are adaptable to complex reasoning types. Particularly a single approach that can answer questions with different reasoning types. 



In this paper, we present a modular approach called \textbf{\system}~(\textbf{Sy}stem for \textbf{G}eneralizable and \textbf{M}odular question \textbf{A}nswering over knowledge bases), that is built on a framework adaptable to different KB representations and reasoning types. \system~ introduces intermediate representations based on lambda calculus to adapt to new reasoning types and representations. \system~, following the recent advances in KBQA such as NSQA~\cite{pavan2020} and ReTraCk~\cite{chen-etal-2021-retrack}, is a modular approach with independent Abstract Meaning Representation, Entity Linking, and Relation Linking modules. In contrast to NSQA which is tuned specifically to DBpedia-based KBQA datasets, \system~is generalizable to multiple knowledge bases and multiple reasoning types. In order to evaluate our generalizable approach, we consider datasets that have: (a) DBpedia and Wikidata as knowledge bases, and (b) multi-hop and temporal as the reasoning types. 

In pursuit of this goal, we also address the lack of temporal reasoning datasets on knowledge bases that we are considering in this work, specifically Wikidata. We annotate and create \dataset; a Wikidata-based dataset focused on temporal reasoning. \dataset~is a parallel dataset to TempQuestions dataset~\cite{jia2018a} which is a Freebase based temporal reasoning dataset derived from three other datasets \textit{Free917} \cite{cai2013}, \textit{WebQuestions} \cite{berant2013} and \textit{ComplexQuestions} \cite{bao2016}. While the Freebase dataset consists of question answer pairs along with temporal signal classifications, our dataset is annotated with intermediate SPARQL queries enabling evaluation of different modules in a KBQA pipeline. 

%a specific category of questions called \textbf{temporal questions}, where answering a question requires reasoning about points and intervals in time. For example, to answer the question \textit{What team did Joe Hart play for before Man City?}, the system must retrieve or infer \textit{when} Joe Hart played for Man City, \textit{when} Joe Hart played for other teams, and which of the latter intervals occurred \textit{before} the former.

%\vspace{-0.2cm}
\begin{table}[htb]
\begin{small}
\centering
\begin{tabular}{l|l}
\toprule
% \hline
\begin{tabular}[l]{@{}l@{}}
    \textbf{Category}\\
\end{tabular} 
& 
\textbf{Example} \\
\midrule
% \hline

\begin{tabular}[l]{@{}l@{}}
    Single-Hop
\end{tabular} 
& 

\begin{tabular}[c]{@{}l@{}}

\emph{ Who directed Titanic Movie?}\\
{\bf SPARQL:}
select distinct ?a where \{\\
  wd:Q44578 wdt:P57 ?a\}\\

    \end{tabular} \\
\hline
\begin{tabular}[l]{@{}l@{}}
    Multi-hop\\
\end{tabular} 
& 

\begin{tabular}[c]{@{}l@{}}

\emph{ Which movie is directed by James Cameron }\\
\emph{ starring Leonardo DiCaprio?  }\\
{\bf SPARQL:}
select distinct ?a where \\
  \{?a wdt:P57 wd:Q42574. \\
  ?a wdt:P161 wd:Q38111. \} \\
   \end{tabular} \\
\hline
\begin{tabular}[l]{@{}l@{}}
    Temporal
\end{tabular} 
& 
\begin{tabular}[c]{@{}l@{}}
\emph{ Who was the US President }\\
\emph{ during cold war?  }{\bf SPARQL:}
in Figure~\ref{fig:example} \\
\end{tabular} \\
\bottomrule
\end{tabular}
\caption{Examples of Single-hop, Multi-hop and Temporal reasoning questions on Wikidata.}
%\vspace{-0.2cm}
\label{tab:multi-hop}
\end{small}
\end{table}


%Therefore, clearly demonstrating the need for extending approaches for other types of reasoning such as temporal and spatial. 
%In order to extend the scope of reasoning in KBQA, 
%This needs understanding of the question in terms of the knowledge as available in the KB. In specific, they map question to a KB-specific query, that when executed over the KB would derive the answer \cite{berant2013, svitlana2019, pavan2020}. 
%For this they: 1) map terms in the question to KB elements (i.e., entities and predicates) and 2) perform reasoning to infer answer from the facts as in the KB. Different questions have different reasoning requirements, depending upon the question complexity and the available KB facts. For example, possible KB-specific queries for question \textit{Country of Obama's birth?} include \textit{birthCountry("Obama", ?X)} or \textit{birthCity("Obama", ?Y) \& locatedIn(?Y, ?X)}. The $2^{nd}$ query performs multi-hop reasoning. 
%In this paper, we present a KBQA dataset focused on \textbf{temporal questions}, where reasoning to derive answers involve at least one step of temporal reasoning \cite{jia2018a, jia2018b} i.e., a manipulation of time intervals of the associated events. For example, as shown in Table~\ref{tab:temporal_reasoning_example}, the question \textit{What team did Joe Hart play for before Man City?}, requires knowing the time intervals of teams which Joe Hart played for and picking the one just before Man City.
%\textit{Who became president of France after ww2?}.


 
%Temporal Question Answering over knowledge bases is heavily impacted by the lack of datasets for evaluating the systems. 
%\vspace{-0.2cm}
%Progress on Temporal KBQA is hindered by a lack of  datasets that can truely assess temporal reasoning capability of existing KBQA systems. To the best of our knowledge, \textit{TempQuestions}~\cite{jia2018a} is the only available dataset for evaluating purely this aspect. It  has, however, a number of drawbacks: (a) the dataset uses Freebase~\cite{freebase} as the knowledge base, which is no longer maintained and  was officially discontinued in $2014$~\cite{freebase}; (b) the dataset contains only question-answer pairs and not their intermediate SPARQL queries which could be useful in  evaluating interpretability aspect of KBQA approaches based on semantic parsing ~\cite{yih2014semantic}; (c) unlike regular KBQA datasets~\cite{lcquad2, swq, azmy-etal-2018-farewell} that can attest KBQA generality over multiple knowledge bases such as DBpedia, and Wikidata, \textit{TempQuestions} is suited for a single KB.% In particular, to the best of our knowledge, there is no benchmark dataset for temporal questions with parallel annotations on multiple KBs.

%Past work on KBQA vary in terms of the core approach being used, that range from dependency parse-based approaches \cite{zou2014, sun2020b} to those involving end-to-end learning \cite{sun2020a, verga2020}. Many of these approaches use single KB as their knowledge source. Moreover, many of the datasets used for evaluation of these approaches are also single KB specific, such as Freebase or DBpedia. These factors are likely to have limited the generalizability of those approaches to other KBs \cite{dennis2018}. New datasets have recently been released with parallel annotations on multiple KBs \cite{lcquad2, swq, webqsp}, thus offering opportunity for generalizability across KBs. However, such datasets for complex questions are rare. 
 %Our aim in this paper is to fill the above mentioned gaps by adapting the \textit{TempQuestions} dataset to Wikidata and by enhancing it with additional SPARQL query annotations. %Specifically, since \textit{TempQuestions} dataset contains complex temporal reasoning questions but on Freebase, we reused the natural language questions to create a temporal qa dataset  for WikiData~\cite{} as the Knowledge Base.
 %This would easily serve the purpose of building a dataset with parallel annotations on multiple KBs (in our case two different KBs, i.e.,WikiData and Freebase). 
% Having SPARQL queries for temporal dataset is crucial to refresh ground truth answers as the KB evolves.
%We choose Wikidata for this dataset because it is well structured, fast evolving, and the most up-to-date KB, making it a suitable candidate for temporal KBQA.
%Our resulting dataset thus contains parallel annotations (on both Wikidata and Freebase). This will help drive research towards development of generalizable approaches, i.e., those that could be easily be adaptable to multiple KBs.
%In order to encourage development of interpretable, semantic parsing-based approaches, we (1) annotate the questions with SPARQL queries and answers over Wikidata, and (2) annotate a subset of this dataset with intermediate representations for the entities, relations, $lambda$-expression along with SPARQL needed to answer the question.
%with information necessary for evaluating entity linking, relation linking, and intermediate sparql representation that are necessary components of a KBQA system.  

 
 %a subset of this dataset is also annotated with outputs expected at various intermediate stages of the pipeline.

%In this paper, we also describe a neuro-symbolic approach to temporal KBQA. Although, primary goal of this approach is to simply serve baseline for the dataset described above, it has design level novelty guided by the requirements of interpretability and generalizability\pavan{I dont think we evaluate this aspect so calling it out as novelty might not be the best idea}. It includes a novel question understanding framework, where an intermediate KB-agnostic logic representation of the question is obtained first, followed by mapping onto a KB-specific logic representation that further could be executed over KB as SPARQL queries.

In summary, the main contributions of this paper are:
%\vspace{-0.2cm}

\begin{itemize}
      \item A modular, generalizable approach, called \system, for KBQA with lambda calculus based intermediate representations that enable adaptation to: (a) multiple knowledge bases, specifically DBpedia and Wikidata, and (b) multiple reasoning types such as multi-hop and temporal reasoning. 
     \item A benchmark dataset, called \dataset, for building temporal-aware KBQA systems on \textit{Wikidata} with parallel annotations on \textit{Freebase}. 
    %  , thus encouraging the development of approaches for temporal KBQA that generalize across KBs.
    \item Experimental results show \system~ achieves state-of-the-art numbers on LC-QuAD 1.0, WebQSP-WD, and comparable numbers on QALD-9 dataset. We also present baseline numbers for Simple WebQuestions and new dataset introduced in this paper; \dataset.
%{\color{red}Contributions on the performance.}
 \end{itemize}

%We first give details of the benchmark dataset in the next section, and then we describe baseline neuro-symbolic approach in the following section, followed further by discussions on experimentation and results.

%This involves understanding the NL question in terms of knowledge as available in the KB, in order to map that to a KB-specific query that when executed over the KB would derive the answer \cite{}. Depending upon the question complexity, this involves: 1) mapping of terms in the question onto KB elements (i.e., entities and predicates) and 2) reasoning to infer answer from the facts as found in the KB. For example, depending upon facts available in the KB, KB-specific queries for question \textit{Did Zinedine win 1998 football worldcup?} could be \textit{PersonWon("Zinedine Zidane", "1998 FIFA Worldcup")} or \textit{TeamMember("Zinedine Zidane", a) \& TeamWon(a, "1998 FIFA Worldcup")}. Reasoning in case of second query is multi-hop reasoning. % where facts considered to answer the question are inferred through composition of pairs of facts in the KB that are linked through common entity.
%Depending upon the type of the fact inferred, the reasoning step could be categorized as temporal, spatial and so on. For example, answering question \textit{Who became president of France after ww2?} would need temporal reasoning involving manipulation using time intervals. % since answer derivation would require looking into the time intervals of all the French presidents and choosing the one whose time interval is immediately after the time interval of 'World War 2'. 
%In this paper, our focus in on such kind of questions, called temporal questions, where at least one step of temporal reasoning is needed to derive the answer \cite{}.
%focus of this paper is on temporal question. 

%Past work on KBQA vary in terms complexity of the questions being addressed, with recent approaches addressing more complex questions. Recent work on temporal-specific KBQA include \cite{}. Past work also vary in terms of the core approach being adopted, ranging from dependency parse-based approaches to those involving end-to-end learning \cite{}. However, many of these approaches have focused on using single KB as their knowledge source \cite{}. Moreover, many of the datasets used for evaluation of these approaches are also single KB specific, such as Freebase or DBPedia \cite{}. These factors are likely to have resulted in limitations in the approach in terms of generalizability to other KBs. However, recently there are datasets made available with parallel annotations on multiple KBs, thus offering opportunities to explore KBQA approaches that are generalizable across KBs. But these cover only less complex questions. In particular, to our knowledge, there is no benchmark dataset for temporal questions with parallel annotations on multiple KBs. Our aim in this paper is to address this gap. In addition, in order to encourage the development of interpretable approaches, a subset of this dataset is also annotated with outputs expected at various intermediate stages of the pipeline.

%In this paper, we also describe a neuro-symbolic approach to temporal KBQA. The goal is to have this approach serve as a baseline approach for the dataset described above. With interpretability and generalizability being the guiding factors, this approach includes a question understanding framework where an intermediate KB-agnostic logic representation of the question is obtained first, followed by mapping onto a KB-specific logic representation that further could be executed over KB after mapping onto corresponding SPARQL queries.

%In the next section, we describe the benchmark dataset that we introduce. Then we describe the describe the neuro-symbolic approach that serve as a baseline for the dataset introduced. Followed by discussion on experimentation and results.

%One striking common feature of most of these approaches is that they are all built with goal of using a single KB (such as Freebase or DbPedia) as their knowledge source. As a result, it is hard to adapt models built using of these approaches to work on KBs other than what they are built for. In addition, datasets used to evaluate these approaches are also typically built using a single KB as knowledge source. On the other hand, datasets that  encourage development of approaches that are generalizable to multiple KBs with minimal effort  are highly desirable. In this paper, we present a benchmark dataset built towards this goal. In specific, we took a dataset that is built for Freebase and adapted a subset of that to build a parallel dataset for Wikidata. Existence of such dataset with parallel annotations would facilitate development of generalizable KGQA approaches that work on more than one KB. In addition, to encourage development of interpretable approaches we have annotated the dataset with outputs expected at intermediate various stages of the pipeline. In this paper we have chosen to focus on temporal question, and our plan is to extend this effort in the future to beyond temporal questions.




==> TempQA-AAAI2022(2)/text/related_work.tex <==
\section{Related Work}

\begin{table*}
\centering
\resizebox{2\columnwidth}{!}{%
\begin{tabular}{l|l|l|c|c|c}
\toprule
\textbf{Datasets} & \textbf{Knowledge Base} & \textbf{Emphasis} & \textbf{SPARQL} & \textbf{Intermediate} & \textbf{Templates}\\
 &  &  & \textbf{} &  \textbf{Evaluation} & \\ 
\midrule  
QALD-9 & DBpedia & Multi-hop & \cmark & \cmark & \xmark \\
LC-QuAD 1.0 & DBpedia & Multi-hop & \cmark & \cmark & \cmark \\
LC-QuAD 2 & DBpedia, Wikidata & Multi-hop & \cmark & \cmark & \cmark \\
Simple Questions & Freebase, DBpedia, Wikidata & Single-hop & \cmark & \cmark & \xmark \\
Web Questions & Freebase
& Multi-hop
& \xmark
& \xmark
& \xmark \\
WebQSP
& Freebase, Wikidata
& Multi-hop
& \cmark
& \cmark
& \xmark \\
Complex Web Questions
& Freebase
& Multi-hop
& \xmark
& \xmark
& \xmark \\
TempQuestions
& Freebase
& Temporal
& \xmark
& \xmark
& \xmark \\
\midrule
\midrule
\textbf{\dataset}
& \textbf{Freebase, Wikidata}
& \textbf{Temporal}
& \cmark
& \cmark
& \xmark \\
\bottomrule
\end{tabular}
}
\caption{This table compares most of the KBQA datasets based on features relevant to the work presented in this paper. References: QALD-9~\cite{QALD_2017}, LC-QuAD 1.0~\cite{trivedi2017lc}, LC-QuAD 2.0~\cite{lcquad2}, Simple Questions~\cite{journals/corr/BordesUCW15}, Web Questions~\cite{berant2013}, Web Questions-SP~\cite{cai2013}, Complex Web Questions~\cite{talmor18compwebq}, TempQuestions \cite{jia2018a}}
\label{tab:related_work_datasets}
\end{table*}
%\vspace{-0.5cm}

{\bf KBQA Datasets:} Over the years,  many  question answering datasets have been developed for KBQA, such as Free917~\cite{cai2013}, SimpleQuestions~\cite{journals/corr/BordesUCW15}, WebQuestions~\cite{berant2013}, QALD-9~\cite{QALD_2017}, LC-QuAD 1.0~\cite{trivedi2017lc}, and LC-QuAD 2.0~\cite{lcquad2}. In Table~\ref{tab:related_work_datasets}, we compare each of these datasets across the following features: (a) underlying KB, including subsequent extensions, e.g. Wikidata~\cite{wikidata-benchmark} and DBpedia~\cite{azmy-etal-2018-farewell} based versions of SimpleQuestions, as well as the Wikidata subset of WebQSP ~\cite{webqsp}; %The underlying knowledge base: this includes the original knowledge base that the dataset was based on (e.g. Freebase for SimpleQuestion) and also the efforts to create parallel datasets that work on multiple KBs (e.g. Wikidata~\cite{wikidata-benchmark} and DBpedia~\cite{azmy-etal-2018-farewell} based versions of SimpleQuestions). 
%Similarly, WebQSP has a subset mapped to Wikidata~\cite{webqsp}. 
%(b) Reasoning types: the different reasoning types the dataset is attesting; e.g. single-hop, multi-hop or temporal reasoning. %As Table~\ref{tab:related_work_datasets} shows, most datasets focus of single-hop and multi-hop reasoning;
(b) reasoning types that are emphasized in the dataset;
(c) availability of SPARQL queries, entities, and relationships for intermediate evaluation; and (d) the use of question templates, which can often generate noisy, unnatural questions.
%Template-based datasets provide an option to generate a lot of data with sometimes significant noise in comparison to non-template based that are carefully curated. 
As Table~\ref{tab:related_work_datasets} shows, our dataset is distinguished from prior work in its emphasis on temporal reasoning, its application to both Freebase and Wikidata, and its annotation of intermediate representations and SPARQL queries. 

%These datasets focus on single hop and multi-hop questions ignoring complex reasoning questions. While~\cite{QALD_2017} are natural questions with SPARQL queries manually annotated,~\cite{lcquad2, trivedi2017lc} are template based datasets that allows creating of large question-sparql-answer triplets facilitating training of data hungry models for KBQA~\cite{}. 

%Not all datasets  


%Many of these are used in building semantic parsing capabilities to get the logic form closer to Freebase. ~\cite{bao-etal-2016-constraint} introduced another benchmark called ComplexQuestions on Freebase to test the multi-constraint questions. 

%Closest to our benchmark, TempQuestions~\cite{jia2018a} is constructed by gathering questions which have temporal signals from the Free917, WebQuestions, and ComplexQuestions datasets, resulting in 1272 temporal questions. As mentioned in Section~\ref{sec:intro}, we reuse the TempQuestions dataset by mapping the answers to Wikidata and annotating them with SPARQL queries that can be run on Wikidata.
The most relevant KBQA dataset to our work is TempQuestions~\cite{jia2018a}, upon which we base \dataset, as  described in Section \ref{sec:dataset}.

%QALD\footnote{http://qald.aksw.org/} is another set of datasets that were developed over years to test the QA capabilities of QA systems over DBPedia KB. Among these QALD-7~\cite{QALD_2017} introduced a small test set on Wikidata as well. Template based datasets are introduced in LC-Quad-1.0~\cite{trivedi2017lc} and LC-Quad-2.0~\cite{dubey2017lc2}. LC-Quad-2.0 has parallel annotaitons for both DbPedia and Wikidata.

{\bf KBQA Systems:} %ACCU~\cite{accu} and QUINT~\cite{quint} are two end-to-end systems that work on Freebase. TEQUILA~\cite{jia2018b} use these systems as baselines and generates answers for the simple questions generated from their framework. It then applies temporal reasoning on top of these answers to generate the final answer. 
%Due to lack of enough training data, many graph driven/rule based systems have been proposed over the last few years. 
Specific to TempQuestions, the TEQUILA~\cite{jia2018b} system uses existing end-to-end Freebase KBQA systems (AQQU~\cite{accu} and QUINT~\cite{quint}) to generate answers to simple questions, upon which it applies temporal reasoning to arrive at a final answer. 
In general, many graph driven/rule-based KBQA systems have been proposed to address datasets with fewer training data ~\cite{diefenbach2017wdaqua,zou2014natural,mazzeo2016answering,vakulenko2019message}. 
In contrast, end-to-end deep learning systems have demonstrated some success~\cite{yih2014semantic,xu2016question,bao2016constraint,yu2017improved,wu2019general,bordes2015large,xu2019enhancing,hu2018state,zheng2019question}.
%On the other hand,  numerous deep learning based systems developed over years for the KBQA task~\cite{yih2014semantic,xu2016question,bao2016constraint,yu2017improved,wu2019general,bordes2015large,xu2019enhancing,hu2018state,zheng2019question}.
Recently, there have been efforts to build explainable KBQA systems~\cite{pavan2020,singh2018frankenstein,liang2021querying}. We build on top of these representational efforts and introduce a baseline using $\lambda$-expressions with the required additional functions.\\ 

%{\bf Semantic Parsing:} Parsing natural language questions in the context of KBQA and representing them into an intermediate logic form is carried out in works~\cite{pavan2020,yih-etal-2016-value,cao-etal-2019-semantic,berant2013,liang-etal-2013-learning,wang-etal-2015-building,zhang-etal-2017-macro,pasupat-liang-2016-inferring,10.5555/286695}. 

==> TempQA-AAAI2022(2)/text/related_work_pavan.tex <==
\section{Related Work}
\begin{table*}
\centering
\resizebox{2\columnwidth}{!}{%
\begin{tabular}{l|l|l|c|c|c}
\toprule
\textbf{Datasets} & \textbf{Knowledge Base} & \textbf{Emphasis} & \textbf{SPARQL} & \textbf{Intermediate} & \textbf{Natural questions}\\
 &  &  & \textbf{} &  \textbf{Evaluation} & \\ 
\midrule  
QALD-9 & DBpedia & Multi-hop & \cmark & \cmark & \cmark \\
LC-QuAD 1.0 & DBpedia & Multi-hop & \cmark & \cmark & \xmark \\
LC-QuAD 2 & DBpedia, Wikidata & Multi-hop & \cmark & \cmark & \xmark \\
Simple Questions & Freebase, DBpedia, Wikidata & Single-hop & \cmark & \cmark & \cmark \\
Web Questions & Freebase
& Multi-hop
& \xmark
& \xmark
& \cmark \\
WebQSP
& Freebase, Wikidata
& Multi-hop
& \cmark
& \cmark
& \cmark \\
Complex Web Questions
& Freebase
& Multi-hop
& \xmark
& \xmark
& \cmark \\
TempQuestions
& Freebase
& Temporal
& \xmark
& \xmark
& \cmark \\
\midrule
\midrule
\textbf{\dataset}
& \textbf{Freebase, Wikidata}
& \textbf{Temporal}
& \cmark
& \cmark
& \cmark \\
\bottomrule
\end{tabular}
}
\caption{This table compares most of the KBQA datasets based on features relevant to the work presented in this paper. 
%References: QALD-9~\cite{QALD_2017}, LC-QuAD 1.0~\cite{trivedi2017lc}, LC-QuAD 2.0~\cite{lcquad2}, Simple Questions~\cite{journals/corr/BordesUCW15}, Web Questions~\cite{berant2013}, Web Questions-SP~\cite{cai2013}, Complex Web Questions~\cite{talmor18compwebq}, TempQuestions \cite{jia2018a}
}
\label{tab:related_work_datasets}
\end{table*}
%\vspace{-0.5cm}


{\bf KBQA Systems:} %ACCU~\cite{accu} and QUINT~\cite{quint} are two end-to-end systems that work on Freebase. TEQUILA~\cite{jia2018b} use these systems as baselines and generates answers for the simple questions generated from their framework. It then applies temporal reasoning on top of these answers to generate the final answer. 
%Due to lack of enough training data, many graph driven/rule based systems have been proposed over the last few years. 
KBQA approaches can be primarily categorized into two groups: (a) Question-to-entities: where techniques output the answer entities from the knowledge graph ignoring the SPARQL query~\cite{saxena-etal-2020-improving,sun-etal-2018-open,qamp}, and (b) semantic parsing based: where approaches output intermediate SPARQL queries (or logic forms) that can retrieve the answer from the knowledge base~\cite{singh2018frankenstein,pavan2020,gAnswer}. First, in question-to-entities category,~\cite{qamp} leverages a message passing technique on a two hop graph from the entities mentioned in the question to retrieve answers from the knowledge graph. 
~\cite{saxena-etal-2020-improving} encodes both text and entities, text based on language models and entities based on knowledge graph embeddings~\cite{complexE} and shows that text can help KBQA in an incomplete setting. In contrast to question-to-entities approach, the semantic parsing based approaches improves interpretability and facilitates evaluation of different modules as shown by Frankestein~\cite{singh2018frankenstein}, and NSQA~\cite{pavan2020}. Both, Frankestein~\cite{singh2018frankenstein}, and NSQA~\cite{pavan2020} follow a pipeline based approach with the differentiating factor being the use of Abstract Meaning Representation as a starting point by NSQA. We build on top of these representational efforts and introduce $\lambda$-expressions with the required additional functions for adapting to new knowledge graphs and new reasoning types. 
% whereas the existing approaches lack the ability and are tuned for a single knowledge graph. 

% Specific to TempQuestions, the TEQUILA~\cite{jia2018b} system uses existing end-to-end Freebase KBQA systems (AQQU~\cite{accu} and QUINT~\cite{quint}) to generate answers to simple questions, upon which it applies temporal reasoning to arrive at a final answer. 
% In general, many graph driven/rule-based KBQA systems have been proposed to address datasets with fewer training data ~\cite{diefenbach2017wdaqua,zou2014natural,mazzeo2016answering,vakulenko2019message}. 
% In contrast, end-to-end deep learning systems have demonstrated some success~\cite{yih2014semantic,xu2016question,bao2016constraint,yu2017improved,wu2019general,bordes2015large,xu2019enhancing,hu2018state,zheng2019question}.

%\\ 

%{\bf Semantic Parsing:} Parsing natural language questions in the context of KBQA and representing them into an intermediate logic form is carried out in works~\cite{pavan2020,yih-etal-2016-value,cao-etal-2019-semantic,berant2013,liang-etal-2013-learning,wang-etal-2015-building,zhang-etal-2017-macro,pasupat-liang-2016-inferring,10.5555/286695}. 

{\bf KBQA Datasets:} Over the years,  many  question answering datasets have been developed for KBQA, such as Free917~\cite{cai2013}, SimpleQuestions~\cite{journals/corr/BordesUCW15}, WebQuestions~\cite{berant2013}, QALD-9~\cite{QALD_2017}, LC-QuAD 1.0~\cite{trivedi2017lc}, and LC-QuAD 2.0~\cite{lcquad2}. In Table~\ref{tab:related_work_datasets}, we compare each of these datasets across the following features: (a) underlying KB, including subsequent extensions, e.g. Wikidata~\cite{wikidata-benchmark} and DBpedia~\cite{azmy-etal-2018-farewell} based versions of SimpleQuestions, as well as the Wikidata subset of WebQSP ~\cite{webqsp}; %The underlying knowledge base: this includes the original knowledge base that the dataset was based on (e.g. Freebase for SimpleQuestion) and also the efforts to create parallel datasets that work on multiple KBs (e.g. Wikidata~\cite{wikidata-benchmark} and DBpedia~\cite{azmy-etal-2018-farewell} based versions of SimpleQuestions). 
%Similarly, WebQSP has a subset mapped to Wikidata~\cite{webqsp}. 
%(b) Reasoning types: the different reasoning types the dataset is attesting; e.g. single-hop, multi-hop or temporal reasoning. %As Table~\ref{tab:related_work_datasets} shows, most datasets focus of single-hop and multi-hop reasoning;
(b) reasoning types that are emphasized in the dataset;
(c) availability of SPARQL queries, entities, and relationships for intermediate evaluation; and (d) the use of question templates, which can often generate noisy, unnatural questions.
%Template-based datasets provide an option to generate a lot of data with sometimes significant noise in comparison to non-template based that are carefully curated. 
As Table~\ref{tab:related_work_datasets} shows, our dataset is distinguished from prior work in its emphasis on temporal reasoning, its application to both Freebase and Wikidata, and its annotation of intermediate representations and SPARQL queries. The most relevant KBQA dataset to our work is TempQuestions~\cite{jia2018a}, upon which we base \dataset, as  described in dataset section. CRONQUESTIONS~\cite{DBLP:conf/acl/SaxenaCT20} is another temporal QA dataset proposed recently over a small subset of Wikidata. It has template based questions targeted at temporal KG embeddings and QA.


%These datasets focus on single hop and multi-hop questions ignoring complex reasoning questions. While~\cite{QALD_2017} are natural questions with SPARQL queries manually annotated,~\cite{lcquad2, trivedi2017lc} are template based datasets that allows creating of large question-sparql-answer triplets facilitating training of data hungry models for KBQA~\cite{}. 

%Not all datasets  


%Many of these are used in building semantic parsing capabilities to get the logic form closer to Freebase. ~\cite{bao-etal-2016-constraint} introduced another benchmark called ComplexQuestions on Freebase to test the multi-constraint questions. 

%Closest to our benchmark, TempQuestions~\cite{jia2018a} is constructed by gathering questions which have temporal signals from the Free917, WebQuestions, and ComplexQuestions datasets, resulting in 1272 temporal questions. As mentioned in Section~\ref{sec:intro}, we reuse the TempQuestions dataset by mapping the answers to Wikidata and annotating them with SPARQL queries that can be run on Wikidata.
% The most relevant KBQA dataset to our work is TempQuestions~\cite{jia2018a}, upon which we base \dataset, as  described in Section \ref{sec:dataset}.

%QALD\footnote{http://qald.aksw.org/} is another set of datasets that were developed over years to test the QA capabilities of QA systems over DBPedia KB. Among these QALD-7~\cite{QALD_2017} introduced a small test set on Wikidata as well. Template based datasets are introduced in LC-Quad-1.0~\cite{trivedi2017lc} and LC-Quad-2.0~\cite{dubey2017lc2}. LC-Quad-2.0 has parallel annotaitons for both DbPedia and Wikidata.


==> text/abstract.tex <==
\begin{abstract}
 
 Knowledge Base Question Answering (KBQA) tasks that involve complex reasoning are emerging as an important research direction. However, most of the recent KBQA systems are built towards supporting multi-hop reasoning over a single knowledge base. In this paper, we present a KBQA system that is built with the goal of generalizing across multiple knowledge bases and multiple reasoning types. Our system built as modular pipeline, by keeping interpretability at intermediate stages also as the guiding principle, contains three high level modules: 1) KB-agnostic question understanding module that is common across KBs 2) Ontology module to support additional reasoning types simply by extending the ontology and 3) KB-specific question mapping and answering module to address the KB specific aspects of the answer extraction. We demonstrate effectiveness of our system by evaluating on datasets belonging to two distinct knowledge bases, DBpedia and Wikidata. In addition, to demonstrate extensibility to additional reasoning types we evaluate on a new Temporal KBQA benchmark dataset, named TempQA-WD, introduced in this paper. This dataset is adapted from an old dataset to Wikidata. We show state-of-the-art results achieved on DBpedia based LCQuad and QALD datasets and Wikidata based WebQSP datasets. Additionally, we also present baseline numbers achieved on the new temporal dataset.
 
 %Question Answering of Knowledge Bases has been a long standing problem in the Natural Language Processing domain. The goal of the task is to evaluate systems ability to reason and retrieve an answer from the knowledge base, given the natural language question. 
 
 %Knowledge Base Question Answering (KBQA) tasks that involve complex reasoning are emerging as an important research direction. However, most existing KBQA datasets focus primarily on generic multi-hop reasoning over explicit facts, largely ignoring other reasoning types such as temporal, spatial, and taxonomic reasoning. In this paper, we present a benchmark dataset for temporal reasoning, \dataset, to encourage research in extending the present approaches to target a more challenging set of complex reasoning tasks. Specifically, our benchmark is a temporal question answering dataset with the following advantages: (a) it is based on Wikidata, which is the most frequently curated, openly available knowledge base, (b) it includes intermediate sparql queries to facilitate the evaluation of semantic parsing based approaches for KBQA, and (c) it generalizes to multiple knowledge bases: Freebase and Wikidata. %allows evaluating generalizable temporal KBQA systems on multiple knowledge bases (Freebase and Wikidata);  
 %Including the dataset, we present a modular temporal knowledge base question answering system on Wikidata as a baseline system. Overall, the baseline system shows a performance of XX on the dataset showing significant headroom for research in the temporal reasoning domain.
 %In addition to the new dataset, we present a modular, temporal KBQA system  \system~as a baseline. Overall, the baseline system shows a performance of 0.32 (F1 metric) on the dataset showing significant headroom for research in the temporal reasoning domain.
 
 
 %(b) they target only one knowledge base lacking the ability for the systems to show generalized approaches over multiple knowledge bases; (c) most datasets have question-answer pairs without an intermediate SPARQL representation. \pavan{Both b and c are primarily for Temporal Question Answering.}


 %We describe a benchmark dataset that we release towards facilitating effective evaluation of approaches, and to try address gaps in the existing benchmarks. Our main goal with this dataset is to encourage approaches that are interpretable and generalizable across different knowledge bases and reasoning requirements. In specific, we took an existing temporal question answering (QA) dataset that was built for Freebase and adapted a subset of that to build a parallel dataset for Wikidata. This enables performance evaluation of temporal KBQA approaches simultaneously on more than one knowledge base. In addition we also provide fine-grained annotation on a subset that enable evaluating interpretability of the approach. Apart from the dataset, we also present a neuro-symbolic approach for temporal KBQA that could serve as a baseline approach on this dataset. This approach includes a question understanding framework where an intermediate KB-agnostic logic representation of the question is obtained first, followed by mapping onto a KB-specific logic representation that further could be executed over KB after mapping onto corresponding SPARQL queries. {\pavan{Pavan: 1. KBQA datasets lacks reasoning with most datasets primarily focused on multi-hop reasoning. Need to including more reasoning types for extending research in KBQA. 2. KBQA datasets cover single knowledge bases. There is a need for parallel datasets that can help evaluate generality of approaches on multiple datasets. 3. KBQA datasets with weak supervision push approaches to directly work with the knowledge graph. Having an intermeditate representation such as a SPARQL query would encourage KG-generic semantic parsing.}}
\end{abstract}

==> text/approach/kb-agnostic/algorithm.tex <==
\begin{algorithm}[htb]
\begin{small}
%\footnotesize
 \caption{AMR to $\lambda$-expression}
 \label{alg:amrTolambda}
\SetAlgoLined
\DontPrintSemicolon
%\KwResult{Write here the result }
%\SetKwInput{KwIn}{Input}
%\SetKwInOut{Input}{Input}
%\Input{$amr$: AMR graph}
\SetKwFunction{FMain}{Convert}
\SetKwProg{Fn}{Function}{:}{}
  \Fn{\FMain{$amr\_root$}}{
        $expr = empty\_expr()$\;
        \eIf{$multi\_event(amr\_root)$}
        {
            $amr\_list$ = $break\_amr(amr\_root)$
            $connective$ = $get\_temp\_connective(amr\_root, amr\_list)$
            \For{each $amr$ in $amr\_list$}
            {
                $sub\_expr = Convert(amr)$\;
                append $sub\_expr$ to $expr$\;
            }
            append $connective$ to $expr$\;
        }
        {
            \For{each $child$ in $children(amr\_root)$}
            {
                $child\_expr = Convert(child)$\;
                append $child\_expr$ to $expr$\;
            }
            $expr = get\_expr(amr\_root, expr)$\;
            %append $e$ to $expr$\;
        }
        \KwRet $expr$\;
  }
  \end{small}
\end{algorithm}

==> text/approach/kb-agnostic/entity_relation_extraction.tex <==
\subsubsection{Entity and Relation Extraction:}
\label{sec:entity-rel-ext}
%The goal here is to spot mentions of entities and relations in the question. 
We use AMR mentions as entity mentions and Propbank frames as relation mentions.
%We extract those directly from the AMR as they are already encoded in AMR as nodes and edges.
%Our system make use of AMR to detect entities and relationships of questions. 
%AMR marks entity surface forms detected in the question text as sink nodes in the AMR graph with quotes mark. Relationships are captured by %Proposition Bank or 
%PropBank Frames AMR nodes. PropBank frame nodes denotes relationship between its children node. %In relationship detection, 
We handle all cases of PropBank frame nodes with arity less than 3 and partially handle 3 or more arity cases. %However, we have observed that there are small number of instances where PropBank node falls in unhandled category. But we'll generalize it and work on these cases in future.

==> text/introduction.tex <==
\section{Introduction}
\label{sec:intro}
%Given a natural language question, the goal of Knowledge Base Question Answering (KBQA) systems is to reason and retrieve the answer based on the facts available in Knowledge Bases (KB). 
The goal of Knowledge Base Question Answering (KBQA) systems is to answer natural language questions by retrieving and reasoning over facts in Knowledge Base (KB).
While reasoning in KBQA is evolving as an important research direction, most existing datasets and research in this area have primarily focused on one-triple questions~\cite{bordes2015large} or multi-hop reasoning questions~\cite{lcquad2,berant2013} as illustrated in Table~\ref{tab:multi-hop}. 
Currently, there is a lack of approaches and datasets that address other types of complex reasoning, such as temporal and spatial reasoning.
In this paper, we focus on a specific category of questions called \textbf{temporal questions}, where answering a question requires reasoning about points and intervals in time. 
For example, to answer the question \textit{What team did Joe Hart play for before Man City?}, the system must retrieve or infer \textit{when} Joe Hart played for Man City, \textit{when} Joe Hart played for other teams, and which of the latter intervals occurred \textit{before} the former.

%\vspace{-0.2cm}
\begin{table}[htb]
\begin{small}
\centering
\begin{tabular}{|l|l|}
%\toprule
\hline
\begin{tabular}[l]{@{}l@{}}
    \textbf{Category}\\
\end{tabular} 
& 
\textbf{Example} \\
%\midrule
\hline

\begin{tabular}[l]{@{}l@{}}
    Single-Hop
\end{tabular} 
& 

\begin{tabular}[c]{@{}l@{}}

\emph{ Who directed Titanic Movie?}\\
{\bf SPARQL:}
select distinct ?a where \{\\
  wd:Q44578 wdt:P57 ?a\}\\

    \end{tabular} \\
\hline
\begin{tabular}[l]{@{}l@{}}
    Multi-hop\\
\end{tabular} 
& 

\begin{tabular}[c]{@{}l@{}}

\emph{ Which movie is directed by James Cameron }\\
\emph{ starring Leonardo DiCaprio?  }\\
{\bf SPARQL:}
select distinct ?a where \{\\
  ?a wdt:P57 wd:Q42574. \\
  ?a wdt:P161 wd:Q38111. \} \\
   \end{tabular} \\
\hline
\begin{tabular}[l]{@{}l@{}}
    Temporal
\end{tabular} 
& 
\begin{tabular}[c]{@{}l@{}}
\emph{ what team did joe hart play }\\
\emph{ for before man city?  }\\
{\bf SPARQL:}
in Figure~\ref{fig:example} \\
\end{tabular} \\
%\bottomrule
\hline
\end{tabular}
\caption{Examples of Single-hop, Multi-hop and Temporal reasoning questions on Wikidata.}
%\vspace{-0.2cm}
\label{tab:multi-hop}
\end{small}
\end{table}


%Therefore, clearly demonstrating the need for extending approaches for other types of reasoning such as temporal and spatial. 
%In order to extend the scope of reasoning in KBQA, 
%This needs understanding of the question in terms of the knowledge as available in the KB. In specific, they map question to a KB-specific query, that when executed over the KB would derive the answer \cite{berant2013, svitlana2019, pavan2020}. 
%For this they: 1) map terms in the question to KB elements (i.e., entities and predicates) and 2) perform reasoning to infer answer from the facts as in the KB. Different questions have different reasoning requirements, depending upon the question complexity and the available KB facts. For example, possible KB-specific queries for question \textit{Country of Obama's birth?} include \textit{birthCountry("Obama", ?X)} or \textit{birthCity("Obama", ?Y) \& locatedIn(?Y, ?X)}. The $2^{nd}$ query performs multi-hop reasoning. 
%In this paper, we present a KBQA dataset focused on \textbf{temporal questions}, where reasoning to derive answers involve at least one step of temporal reasoning \cite{jia2018a, jia2018b} i.e., a manipulation of time intervals of the associated events. For example, as shown in Table~\ref{tab:temporal_reasoning_example}, the question \textit{What team did Joe Hart play for before Man City?}, requires knowing the time intervals of teams which Joe Hart played for and picking the one just before Man City.
%\textit{Who became president of France after ww2?}.


 
%Temporal Question Answering over knowledge bases is heavily impacted by the lack of datasets for evaluating the systems. 
%\vspace{-0.2cm}
Progress on Temporal KBQA is hindered by a lack of  datasets that can truely assess temporal reasoning capability of existing KBQA systems.
To the best of our knowledge, \textit{TempQuestions}~\cite{jia2018a} is the only available dataset for evaluating purely this aspect. It  has, however, a number of drawbacks: (a) the dataset uses Freebase~\cite{freebase} as the knowledge base, which is no longer maintained and  was officially discontinued in $2014$~\cite{freebase}; (b) the dataset contains only question-answer pairs and not their intermediate SPARQL queries which could be useful in  evaluating interpretability aspect of KBQA approaches based on semantic parsing ~\cite{yih2014semantic}; (c) unlike regular KBQA datasets~\cite{lcquad2, swq, azmy-etal-2018-farewell} that can attest KBQA generality over multiple knowledge bases such as DBpedia, and Wikidata, \textit{TempQuestions} is suited for a single KB.% In particular, to the best of our knowledge, there is no benchmark dataset for temporal questions with parallel annotations on multiple KBs.

%Past work on KBQA vary in terms of the core approach being used, that range from dependency parse-based approaches \cite{zou2014, sun2020b} to those involving end-to-end learning \cite{sun2020a, verga2020}. Many of these approaches use single KB as their knowledge source. Moreover, many of the datasets used for evaluation of these approaches are also single KB specific, such as Freebase or DBpedia. These factors are likely to have limited the generalizability of those approaches to other KBs \cite{dennis2018}. New datasets have recently been released with parallel annotations on multiple KBs \cite{lcquad2, swq, webqsp}, thus offering opportunity for generalizability across KBs. However, such datasets for complex questions are rare. 
 Our aim in this paper is to fill the above mentioned gaps by adapting the \textit{TempQuestions} dataset to Wikidata and by enhancing it with additional SPARQL query annotations. %Specifically, since \textit{TempQuestions} dataset contains complex temporal reasoning questions but on Freebase, we reused the natural language questions to create a temporal qa dataset  for WikiData~\cite{} as the Knowledge Base.
 %This would easily serve the purpose of building a dataset with parallel annotations on multiple KBs (in our case two different KBs, i.e.,WikiData and Freebase). 
 Having SPARQL queries for temporal dataset is crucial to refresh ground truth answers as the KB evolves.
We choose Wikidata for this dataset because it is well structured, fast evolving, and the most up-to-date KB, making it a suitable candidate for temporal KBQA.
Our resulting dataset thus contains parallel annotations (on both Wikidata and Freebase). This will help drive research towards development of generalizable approaches, i.e., those that could be easily be adaptable to multiple KBs.
In order to encourage development of interpretable, semantic parsing-based approaches, we (1) annotate the questions with SPARQL queries and answers over Wikidata, and (2) annotate a subset of this dataset with intermediate representations for the entities, relations, $lambda$-expression along with SPARQL needed to answer the question.
%with information necessary for evaluating entity linking, relation linking, and intermediate sparql representation that are necessary components of a KBQA system.  

 
 %a subset of this dataset is also annotated with outputs expected at various intermediate stages of the pipeline.

%In this paper, we also describe a neuro-symbolic approach to temporal KBQA. Although, primary goal of this approach is to simply serve baseline for the dataset described above, it has design level novelty guided by the requirements of interpretability and generalizability\pavan{I dont think we evaluate this aspect so calling it out as novelty might not be the best idea}. It includes a novel question understanding framework, where an intermediate KB-agnostic logic representation of the question is obtained first, followed by mapping onto a KB-specific logic representation that further could be executed over KB as SPARQL queries.

The main contributions of this work are as follows:
%\vspace{-0.2cm}

\begin{itemize}
     
     \item A benchmark dataset, called \dataset, for building temporal-aware KBQA systems on \textit{Wikidata} with parallel annotations on \textit{Freebase}, thus encouraging the development of approaches for temporal KBQA that generalize across KBs.
    \item SPARQL queries for all questions in our benchmark, with a subset of the data also annotated with expected outputs from intermediate stages of the question answering process, i.e. entity and relation linking gold outputs. The goal here is to encourage interpretable approaches that can generate intermediate outputs matching those fine-grained annotations. 
   \item A modular baseline approach, called \system, for temporal QA with novel question understanding framework to serve as a baseline for the benchmark dataset.
 \end{itemize}

%We first give details of the benchmark dataset in the next section, and then we describe baseline neuro-symbolic approach in the following section, followed further by discussions on experimentation and results.

%This involves understanding the NL question in terms of knowledge as available in the KB, in order to map that to a KB-specific query that when executed over the KB would derive the answer \cite{}. Depending upon the question complexity, this involves: 1) mapping of terms in the question onto KB elements (i.e., entities and predicates) and 2) reasoning to infer answer from the facts as found in the KB. For example, depending upon facts available in the KB, KB-specific queries for question \textit{Did Zinedine win 1998 football worldcup?} could be \textit{PersonWon("Zinedine Zidane", "1998 FIFA Worldcup")} or \textit{TeamMember("Zinedine Zidane", a) \& TeamWon(a, "1998 FIFA Worldcup")}. Reasoning in case of second query is multi-hop reasoning. % where facts considered to answer the question are inferred through composition of pairs of facts in the KB that are linked through common entity.
%Depending upon the type of the fact inferred, the reasoning step could be categorized as temporal, spatial and so on. For example, answering question \textit{Who became president of France after ww2?} would need temporal reasoning involving manipulation using time intervals. % since answer derivation would require looking into the time intervals of all the French presidents and choosing the one whose time interval is immediately after the time interval of 'World War 2'. 
%In this paper, our focus in on such kind of questions, called temporal questions, where at least one step of temporal reasoning is needed to derive the answer \cite{}.
%focus of this paper is on temporal question. 

%Past work on KBQA vary in terms complexity of the questions being addressed, with recent approaches addressing more complex questions. Recent work on temporal-specific KBQA include \cite{}. Past work also vary in terms of the core approach being adopted, ranging from dependency parse-based approaches to those involving end-to-end learning \cite{}. However, many of these approaches have focused on using single KB as their knowledge source \cite{}. Moreover, many of the datasets used for evaluation of these approaches are also single KB specific, such as Freebase or DBPedia \cite{}. These factors are likely to have resulted in limitations in the approach in terms of generalizability to other KBs. However, recently there are datasets made available with parallel annotations on multiple KBs, thus offering opportunities to explore KBQA approaches that are generalizable across KBs. But these cover only less complex questions. In particular, to our knowledge, there is no benchmark dataset for temporal questions with parallel annotations on multiple KBs. Our aim in this paper is to address this gap. In addition, in order to encourage the development of interpretable approaches, a subset of this dataset is also annotated with outputs expected at various intermediate stages of the pipeline.

%In this paper, we also describe a neuro-symbolic approach to temporal KBQA. The goal is to have this approach serve as a baseline approach for the dataset described above. With interpretability and generalizability being the guiding factors, this approach includes a question understanding framework where an intermediate KB-agnostic logic representation of the question is obtained first, followed by mapping onto a KB-specific logic representation that further could be executed over KB after mapping onto corresponding SPARQL queries.

%In the next section, we describe the benchmark dataset that we introduce. Then we describe the describe the neuro-symbolic approach that serve as a baseline for the dataset introduced. Followed by discussion on experimentation and results.

%One striking common feature of most of these approaches is that they are all built with goal of using a single KB (such as Freebase or DbPedia) as their knowledge source. As a result, it is hard to adapt models built using of these approaches to work on KBs other than what they are built for. In addition, datasets used to evaluate these approaches are also typically built using a single KB as knowledge source. On the other hand, datasets that  encourage development of approaches that are generalizable to multiple KBs with minimal effort  are highly desirable. In this paper, we present a benchmark dataset built towards this goal. In specific, we took a dataset that is built for Freebase and adapted a subset of that to build a parallel dataset for Wikidata. Existence of such dataset with parallel annotations would facilitate development of generalizable KGQA approaches that work on more than one KB. In addition, to encourage development of interpretable approaches we have annotated the dataset with outputs expected at intermediate various stages of the pipeline. In this paper we have chosen to focus on temporal question, and our plan is to extend this effort in the future to beyond temporal questions.




==> text/related_work.tex <==
\section{Related Work}

\begin{table*}
\centering
\resizebox{2\columnwidth}{!}{%
\begin{tabular}{l|l|l|c|c|c}
\toprule
\textbf{Datasets} & \textbf{Knowledge Base} & \textbf{Emphasis} & \textbf{SPARQL} & \textbf{Intermediate} & \textbf{Templates}\\
 &  &  & \textbf{} &  \textbf{Evaluation} & \\ 
\midrule  
QALD-9 & DBpedia & Multi-hop & \cmark & \cmark & \xmark \\
LC-QuAD 1.0 & DBpedia & Multi-hop & \cmark & \cmark & \cmark \\
LC-QuAD 2 & DBpedia, Wikidata & Multi-hop & \cmark & \cmark & \cmark \\
Simple Questions & Freebase, DBpedia, Wikidata & Single-hop & \cmark & \cmark & \xmark \\
Web Questions & Freebase
& Multi-hop
& \xmark
& \xmark
& \xmark \\
WebQSP
& Freebase, Wikidata
& Multi-hop
& \cmark
& \cmark
& \xmark \\
Complex Web Questions
& Freebase
& Multi-hop
& \xmark
& \xmark
& \xmark \\
TempQuestions
& Freebase
& Temporal
& \xmark
& \xmark
& \xmark \\
\midrule
\midrule
\textbf{\dataset}
& \textbf{Freebase, Wikidata}
& \textbf{Temporal}
& \cmark
& \cmark
& \xmark \\
\bottomrule
\end{tabular}
}
\caption{This table compares most of the KBQA datasets based on features relevant to the work presented in this paper. References: QALD-9~\cite{QALD_2017}, LC-QuAD 1.0~\cite{trivedi2017lc}, LC-QuAD 2.0~\cite{lcquad2}, Simple Questions~\cite{journals/corr/BordesUCW15}, Web Questions~\cite{berant2013}, Web Questions-SP~\cite{cai2013}, Complex Web Questions~\cite{talmor18compwebq}, TempQuestions \cite{jia2018a}}
\label{tab:related_work_datasets}
\end{table*}
%\vspace{-0.5cm}

{\bf KBQA Datasets:} Over the years,  many  question answering datasets have been developed for KBQA, such as Free917~\cite{cai2013}, SimpleQuestions~\cite{journals/corr/BordesUCW15}, WebQuestions~\cite{berant2013}, QALD-9~\cite{QALD_2017}, LC-QuAD 1.0~\cite{trivedi2017lc}, and LC-QuAD 2.0~\cite{lcquad2}. In Table~\ref{tab:related_work_datasets}, we compare each of these datasets across the following features: (a) underlying KB, including subsequent extensions, e.g. Wikidata~\cite{wikidata-benchmark} and DBpedia~\cite{azmy-etal-2018-farewell} based versions of SimpleQuestions, as well as the Wikidata subset of WebQSP ~\cite{webqsp}; %The underlying knowledge base: this includes the original knowledge base that the dataset was based on (e.g. Freebase for SimpleQuestion) and also the efforts to create parallel datasets that work on multiple KBs (e.g. Wikidata~\cite{wikidata-benchmark} and DBpedia~\cite{azmy-etal-2018-farewell} based versions of SimpleQuestions). 
%Similarly, WebQSP has a subset mapped to Wikidata~\cite{webqsp}. 
%(b) Reasoning types: the different reasoning types the dataset is attesting; e.g. single-hop, multi-hop or temporal reasoning. %As Table~\ref{tab:related_work_datasets} shows, most datasets focus of single-hop and multi-hop reasoning;
(b) reasoning types that are emphasized in the dataset;
(c) availability of SPARQL queries, entities, and relationships for intermediate evaluation; and (d) the use of question templates, which can often generate noisy, unnatural questions.
%Template-based datasets provide an option to generate a lot of data with sometimes significant noise in comparison to non-template based that are carefully curated. 
As Table~\ref{tab:related_work_datasets} shows, our dataset is distinguished from prior work in its emphasis on temporal reasoning, its application to both Freebase and Wikidata, and its annotation of intermediate representations and SPARQL queries. 

%These datasets focus on single hop and multi-hop questions ignoring complex reasoning questions. While~\cite{QALD_2017} are natural questions with SPARQL queries manually annotated,~\cite{lcquad2, trivedi2017lc} are template based datasets that allows creating of large question-sparql-answer triplets facilitating training of data hungry models for KBQA~\cite{}. 

%Not all datasets  


%Many of these are used in building semantic parsing capabilities to get the logic form closer to Freebase. ~\cite{bao-etal-2016-constraint} introduced another benchmark called ComplexQuestions on Freebase to test the multi-constraint questions. 

%Closest to our benchmark, TempQuestions~\cite{jia2018a} is constructed by gathering questions which have temporal signals from the Free917, WebQuestions, and ComplexQuestions datasets, resulting in 1272 temporal questions. As mentioned in Section~\ref{sec:intro}, we reuse the TempQuestions dataset by mapping the answers to Wikidata and annotating them with SPARQL queries that can be run on Wikidata.
The most relevant KBQA dataset to our work is TempQuestions~\cite{jia2018a}, upon which we base \dataset, as  described in Section \ref{sec:dataset}.

%QALD\footnote{http://qald.aksw.org/} is another set of datasets that were developed over years to test the QA capabilities of QA systems over DBPedia KB. Among these QALD-7~\cite{QALD_2017} introduced a small test set on Wikidata as well. Template based datasets are introduced in LC-Quad-1.0~\cite{trivedi2017lc} and LC-Quad-2.0~\cite{dubey2017lc2}. LC-Quad-2.0 has parallel annotaitons for both DbPedia and Wikidata.

{\bf KBQA Systems:} %ACCU~\cite{accu} and QUINT~\cite{quint} are two end-to-end systems that work on Freebase. TEQUILA~\cite{jia2018b} use these systems as baselines and generates answers for the simple questions generated from their framework. It then applies temporal reasoning on top of these answers to generate the final answer. 
%Due to lack of enough training data, many graph driven/rule based systems have been proposed over the last few years. 
Specific to TempQuestions, the TEQUILA~\cite{jia2018b} system uses existing end-to-end Freebase KBQA systems (AQQU~\cite{accu} and QUINT~\cite{quint}) to generate answers to simple questions, upon which it applies temporal reasoning to arrive at a final answer. 
In general, many graph driven/rule-based KBQA systems have been proposed to address datasets with fewer training data ~\cite{diefenbach2017wdaqua,zou2014natural,mazzeo2016answering,vakulenko2019message}. 
In contrast, end-to-end deep learning systems have demonstrated some success~\cite{yih2014semantic,xu2016question,bao2016constraint,yu2017improved,wu2019general,bordes2015large,xu2019enhancing,hu2018state,zheng2019question}.
%On the other hand,  numerous deep learning based systems developed over years for the KBQA task~\cite{yih2014semantic,xu2016question,bao2016constraint,yu2017improved,wu2019general,bordes2015large,xu2019enhancing,hu2018state,zheng2019question}.
Recently, there have been efforts to build explainable KBQA systems~\cite{pavan2020,singh2018frankenstein,liang2021querying}. We build on top of these representational efforts and introduce a baseline using $\lambda$-expressions with the required additional functions.\\ 

%{\bf Semantic Parsing:} Parsing natural language questions in the context of KBQA and representing them into an intermediate logic form is carried out in works~\cite{pavan2020,yih-etal-2016-value,cao-etal-2019-semantic,berant2013,liang-etal-2013-learning,wang-etal-2015-building,zhang-etal-2017-macro,pasupat-liang-2016-inferring,10.5555/286695}. 
